Lucid: A Language for Control in the Data Plane

Programmable switch hardware makes it possible to move fine-grained control logic inside the network data plane, improving performance for a wide range of applications. However, applications with integrated control are inherently hard to write in existing data-plane programming languages such as P4. This paper presents Lucid, a language that raises the level of abstraction for putting control functionality in the data plane. Lucid introduces abstractions that make it easy to write sophisticated data-plane applications with interleaved packet-handling and control logic, specialized type and syntax systems that prevent programmer bugs related to data-plane state, and an open-sourced compiler that translates Lucid programs into P4 optimized for the Intel Tofino. These features make Lucid general and easy to use, as we demonstrate by writing a suite of ten different data-plane applications in Lucid. Working prototypes take well under an hour to write, even for a programmer without prior Tofino experience, have around 10x fewer lines of code compared to P4, and compile efficiently to real hardware. In a stateful firewall written in Lucid, we find that moving control from a switch's CPU to its data-plane processor using Lucid reduces the latency of performance-sensitive operations by over 300X.

==> body.tex <==
\section{Evaluation}

\section{Case Studies}

\section{Discussion}

\section{Related Work}

\section{Conclusion}





==> old/appearance_hacks_old.tex <==
% 10pt sigconf weirdness
\captionsetup[figure]{aboveskip=2pt,belowskip=-16pt}
\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
\captionsetup[table]{aboveskip=-14pt,belowskip=4pt}


% VINHACK: make subsubsections great again
\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
  {-0.5\baselineskip \@plus -2\p@ \@minus -.2\p@}%
  {.25\baselineskip}%
  {\ACM@NRadjust\@subsubsecfont}}
\makeatother

% VINHACK: it and sc at the same time
\usepackage{hanging}
\newcommand\fauxsc[1]{\fauxschelper#1 \relax\relax}
\def\fauxschelper#1 #2\relax{%
  \fauxschelphelp#1\relax\relax%
  \if\relax#2\relax\else\ \fauxschelper#2\relax\fi%
}
\def\Hscale{.85}\def\Vscale{.74}\def\Cscale{1.12}
\def\fauxschelphelp#1#2\relax{%
  \ifnum`#1>``\ifnum`#1<`\{\scalebox{\Hscale}[\Vscale]{\uppercase{#1}}\else%
    \scalebox{\Cscale}[1]{#1}\fi\else\scalebox{\Cscale}[1]{#1}\fi%
  \ifx\relax#2\relax\else\fauxschelphelp#2\relax\fi}

\newcommand{\vindef}[2]{
\vspace{4px}
\hangpara{1.5em}{1}
\textit{\fauxsc{#1} ---} #2
\vspace{4px}
}
\newcommand{\btwnvindefs}[0]{\vspace{-4px}}

%VINHACK: circled steps (https://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers)
\definecolor{pennred}{RGB}{149,0,26}
\usepackage{tikz}
\newcommand{\circled}[2][]{%
  \tikz[baseline=(char.base)]{%
    \node[shape = circle, fill = pennred, draw, inner sep = 0pt]
    (char) {\phantom{\ifblank{#1}{#2}{#1}}};%
    \color{white}\footnotesize
    \node at (char.center) {\makebox[0pt][c]{#2}};}}
\robustify{\circled}

% removes footnote with conference info
%\renewcommand\footnotetextcopyrightpermission[1]{} 
% centered X columns
\newcolumntype{Y}{>{\centering\arraybackslash}X}


==> sections/old/challenges.tex <==
\section{Language Challenges}

Developing an application with integrated control for a PISA processor, in particular the Tofino, is very difficult. This is partially because the hardware itself is complex and much different from a general-purpose processor. However, the larger problem is that the available languages and compilers for PISA processors are low level and difficult to use. 

This section describes the three core language-related issues: \emph{missing abstractions}; \emph{implicit constraints}; and \emph{manual optimization}.

\topheading{Missing abstractions.}

\topheading{Implicit constraints.}

\topheading{Manual optimization.}

==> sections/old/compiler.tex <==
\section{The \lang Compiler}

% The \lang compiler translates a \lang program into a correct-by-construction Tofino application, consisting of a Tofino-compatible P4 program plus configurations for all the necessary Tofino components outside the scope of P4. 

\begin{figure}[t]
% \includegraphics[width=.3\linewidth]{figures/seqgraph.pdf}
\includegraphics[width=\linewidth]{figures/compilerhighlevel.pdf}
\caption {Overview of the \lang compiler.}
\vspace{1em}
\label{fig:compileroverview} 
\end{figure}

Figure~\ref{fig:compileroverview} shows the structure and key components of the \lang compiler. The novel part of \lang's front end is its syntactic analysis and type checker, which were described previously. In this section, we describe \lang's back-end, which has three main goals: \textbf{compiling event handlers} into a Tofino-optimized P4 control block; \textbf{translating events and combinators} into P4 code and other Tofino configurations; and \textbf{linking a \lang program} into a native P4 program.

\subsection{Compiling Handlers}
\begin{figure}[t]
\begin{lstlisting}[style=DptBlock]
Array nexthops = new Array<<32>>(NUM_HOSTS);
Array pcts = new Array<<32>>(NUM_PORTS_X3);
Array hcts = new Array<<32>>(NUM_HOSTS);
memop plus(int cur, int x){return cur + x;}

event count_pkt(int dst, int proto);
handle count_pkt (int dst, int proto) {
	int idx = Array.get(nexthops, dst);
	if (proto != TCP) {
		if (proto == UDP)
			idx = idx + NUM_PORTS;
		else 
			idx = idx + NUM_PORTS_X2;
	}
	Array.fset(pcts, idx, plus, 1);		
	if (proto == TCP)
		Array.fset(hcts, dst, plus, 1);
}
\end{lstlisting}
\caption{Counting per-port TCP/UDP packets.}
\label{fig:ctprog}
\end{figure}

% We explain the handler compilation process using the simple handler in Figure~\ref{fig:ctprog} as an example, which counts the number of tcp and udp packets that are sent out of each port.

One key task of \lang's back-end is to translate the handlers of a \lang program into a functionally correct P4 control block that: (1) is functionally correct; (2) compiles to the Tofino; and (3) uses the Tofino's highly parallel architecture efficiently. The compiler does this in two main phases, which we explain by example, using the simple program in Figure~\ref{fig:ctprog}, which counts packets for ports and destinations based on their IP protocol. 

% The general strategy is to first translate into an intermediate 
% representation that conservatively approximates the Tofino's instruction set. Next, the compiler performs dataflow optimizations to both optimize and simplify the program. Finally, we generate a sequence of P4 tables, annotated with Tofino-specific pragmas that aid the Tofino compiler in operating more efficiently. 


\subsubsection{Translating Statements}
After type checking, the \lang compiler front-end reduces the body of a handler into a sequence of primitive statements. The back-end's first task is to translate each primitive statements into P4 code. There are three kinds of primitive statements, each of which maps to P4 according to a different template. 

\heading{Binary operations.} A binary operation evaluate a binary expression over local variables and assign its result to a (possibly new) local variable. The compiler translates a binary operation into a P4 action wrapped with a and table. For example, \inl{idx = idx + NUM_PORTS;} translates to: 
\begin{lstlisting}[style=P4Snip]
action do_idx_eq_0 {idx = idx + NUM_PORTS;}
table idx_eq_0 {	
	actions = {do_idx_eq_0;}
	const default_action = {do_idx_eq_0;}
}
\end{lstlisting}

\heading{Stateful operations.} A Stateful operation is a call to 
a data structure method that operates on a global variable. The compiler translates this call to a table that executes a co-generated \inl{RegisterAction}. The body of the \inl{RegisterAction} is a direct (but verbose) translation of the \inl{memops} passed in the call. For example, here is the register action generated by the call \inl{Array.fset(tcp_cts, port, plus, 1);}.
\begin{lstlisting}[style=P4Snip]
RegisterAction<bit<32>,bit<32>,bit<32>>
  (tcp_cts) fset_1 = {
  void apply(inout bit<32> mem, out bit<32> ret) {
    mem = mem + 1;
  }
};
\end{lstlisting}
The translation from \inl{memop} to \inl{RegisterAction} can be direct because the syntactic restrictions of \inl{memops} guarantees that they can compile to the Tofino's stateful ALUs.


\heading{Branch operations.} A branch operation is an \inl{if}/\inl{else} statement that evaluates a simplified conditional expression. The simplified expression is a conjunction or disjunction of clauses that each compare a local variable with a constant. A branch operation translates to a table that evaluates the conditional expression using ternary rules and calls a true or false action. For example, \inl{if(proto != TCP)} translates to:
\begin{lstlisting}[style=P4Snip]
action if_0_true(); action if_0_false();
table if_0 {	
	keys = {proto : ternary;}
	actions = {if_0_true; if_0_false;}
	entries = {
		(TCP) : if_0_false;
		(_)   : if_0_true;
	}
}
\end{lstlisting}
The compiler also generates a table of this form to select between handlers based on an event ID field. 
% In applications with multiple handlers, this table is placed at the root of the table control graph. 



\begin{figure}[t]
% \includegraphics[width=.3\linewidth]{figures/seqgraph.pdf}
\includegraphics[width=\linewidth]{figures/control_to_dataflow2.pdf}
\caption {Intermediate representations of the program in Figure~\ref{fig:ctprog}. Boxes represent P4 tables that each encapsulate one \lang statement, lines represent either control or data dependencies.}
\label{fig:cttblgraph} 
\end{figure}



\reminder{One thing that we don't mention yet is register allocation for sALUs. We could put that here, but mention that its not reflected in the example because there's only 1 stateful action for each array.}



\subsubsection{Eliminating Control Dependencies}
The templates above give us a way to translate each \lang statement into a primitive P4 table that can implement it on the Tofino. However, if we used these tables directly in a P4 control block, we would end up with a P4 program that used the Tofino's highly-parallel architecture very inefficiently. 

Control dependencies are one core problem. Figure~\ref{fig:cttblgraph}\textbf{(1)} shows a control graph of the compiler-generated primitive tables for the \inl{count_pkt} handler. Implementing this control graph in P4 (i.e., by using \inl{apply} statements to call tables and \inl{switch} statements to branch) would result in a program that took 7 physical stages in the Tofino's pipeline and only executed 1 table and operation in most stages. For contrast, each of the Tofino's stages can execute, in parallel, multiple tables with dozens of arithmetic and comparison operations.

To improve parallelism, the \lang compiler eliminates all control dependencies from the program. The core idea is to transform each primitive table so that it checks all the conditions necessary for its own execution. For example, consider the table \inl{idx_eq_0}. By following the control path from the root node to the table in Figure~\ref{fig:cttblgraph}\textbf{(1)}, we see that it only executes when \inl{(proto != TCP) && (proto != UDP)}. Thus, we transform the table so that it executes a no-op unless these conditions are met. 
\begin{lstlisting}[style=P4Snip]
action do_idx_eq_0 {idx = idx + NUM_PORTS;}
table idx_eq_0 {	
	actions = {do_idx_eq_0;}
	keys = {proto : ternary;}
	entries : { // these entries are ordered.
		(TCP) : do_noop;
		(UDP) : do_noop;
		( _ ) : do_idx_eq_0;
	}
}
\end{lstlisting} 

After transforming all the tables in the program, the \lang compiler performs two optimization passes depicted in Figure~\ref{fig:cttblgraph}\textbf{(2)} and \textbf{(3)}. First, it removes all tables implementing \inl{if/else} statements as those tables only execute empty actions. Second, it disregard all control dependencies and reorders the tables based on dataflow dependencies. At this phase, the \lang-generated P4 control block for the \inl{pkt_ct} handler compiles to 4 stages in the Tofino instead of its original 7. 


\subsubsection{Merging Tables}
The above transformations give us more opportunities to execute tables in parallel. However, the program uses P4 tables inefficiently; each table still only implements one binary or stateful primitive \lang statement. This is fine for simple programs like the \inl{count_pkt} handler, which compiles to only 5 tables. Larger \lang programs can have dozens (or even hundreds) of statements across all of their bodies. The full \exprog, for example, has \reminder{X} statements. 

P4 programs with so many tables are extremely undesirable. Linerate switches can only fit a limited number of physical tables per stage and pipeline. Further, as the number of tables increases, it takes exponentially longer for a P4 compiler to find an efficient mapping of tables to stages~\reminder{}. 

% cite: http://nets.cs.pub.ro/~costin/files/europ4-20-final100.pdf



\begin{figure}[t]
% \includegraphics[width=.3\linewidth]{figures/seqgraph.pdf}
\includegraphics[width=\linewidth]{figures/table_merging_example_pdf.pdf}
\caption {Merged tables for the program in Figure~\ref{fig:ctprog}.\reminder{Todo: compress diagram. Less whitespace.}}
\label{fig:mergedtbls} 
\end{figure}

\begin{figure}[t]
\small
\setlength{\interspacetitleruled}{0pt}%
\setlength{\algotitleheightrule}{0pt}%
\removelatexerror
\begin{algorithm}[H]
\setstretch{.95}
\DontPrintSemicolon


\textcolor{gray}{/* {\footnotesize Global state.}*/}\;


\textcolor{gray}{/* {\footnotesize Main placement algorithm.}*/}\;
\SetKwProg{Fn}{Function}{}{}
\Fn{placePrimitiveTables(primitiveTables):}{
	$\textit{unplaced} \gets \textit{primitiveTables}$\;
	\For{{\bf each} stage {\bf in} stages} {
		\For{{\bf each} table {\bf in} tables} {
			$\textit{stillUnplaced} \gets \textit{[]}$\;
			\For{{\bf each} primitive {\bf in} unplaced} {
	    	    \uIf{canPlace(primative, stage, table);}{

	    	    }
	    	    \Else{
			        $\textit{stillUnplaced.append(primitive)}$\;
			    }
			}
			$\textit{unplaced} \gets \textit{stillUnplaced}$\;

		}
	}	
}
\SetKwProg{Fn}{Function}{}{}
\Fn{canPlace(primitiveTable, stage, table):}{


}



\end{algorithm}
\caption{Pipeline layout algorithm.\reminder{Todo: finish writing up the algo.}}
\label{fig:layoutalgo}
\end{figure}


To reduce the number of tables in emitted code, the penultimate phase of the \lang compiler 
combines the primitive tables into a layout of merged tables that each implement multiple primitive tables. Figure~\ref{fig:mergedtbls} shows how the tables in the example program get laid out. 

The algorithm, listed in Figure~\ref{fig:layoutalgo}, is based on greedy instruction selection. The placement function takes a list of primitive tables to place and two parameters, $M$ and $N$, that define the number of stages in the pipline and the number of tables per stage. For each primitive table, it iterates over all $M$$\cdot$$N$ tables to find the earliest pipeline table that it can merge into, subject to the constraints in Figure~\reminder{X}.

When it finds a table, the placement function calls \reminder{a merge function} that computes a table which implements the cross product of the primitive table and the pipeline table it is being merged into. This merged table replaces the original table in the pipeline. Placement ends when either all primitive tables have been merged into a pipeline table, or the algorithm reaches a primitive table that cannot be placed. 

\subsubsection{Emitting P4}
Based on the layout computed with the above algorithm, the final pass of the compiler emits a control block that contains the pipeline tables, all the objects used by the pipeline tables, and an apply block that calls the pipeline tables in order.

Finally, each pipeline table is annotated with Tofino-specific P4 pragmas. These pragmas are  hints that help the underlying P4 compiler find a better layout. There are two pragmas. 
\begin{itemize}
	\item The \textbf{stage} pragma tells the P4 compiler the earliest pipeline stage where the \lang compiler believes that a table can be placed. The \lang compiler generates this for every pipeline table, based on its stage in the model. 
	\item The \textbf{ignore_dependencies} pragma tells the P4 compiler that it can safely ignore control flow dependencies between pairs of tables. This gives the P4 compiler the freedom to place merged pipeline tables that are in the same stage in the \lang layout into the same stage in the underlying hardware. 
	% This saves us stages. Its important because execution is presumed to be sequential in P4. 
\end{itemize}


\subsection{Compiling Events}
\begin{figure}[t]
\begin{lstlisting}[style=DptBlock]
event a(); event b(); event c(); const GRP = {2, 3};
handle a() {
	generate b();
	mgenerate Event.delay (Event.locate (c(), GRP), 10ms);
}
\end{lstlisting}
\caption{Using \lang's core event abstractions.}
\vspace{1em}
\label{fig:evprog}
\end{figure}

\begin{figure}[t]
	\includegraphics[width=\linewidth]{figures/internaleventdistribution.pdf}
	\caption{Tracing event management for Figure~\ref{fig:evprog}.}
	\label{fig:evtrace}
\end{figure}

\lang's event-based abstractions are enabled by an \emph{event management layer} that sits logically between a \lang application and a native P4 program. This section describes event management by example, using the program in Figure~\ref{fig:evprog} and the execution trace illustrated in Figure~\ref{fig:evtrace}, which represents the distribution of events generated by the handler \inl{a} in the example program. 


\subsubsection{Event Generation} 
We begin in handler \inl{a}, which runs in the ingress match action pipeline and generates two events. 
Each event is stored in a header that includes a location, delay, and event parameters. An event whose location or delay is not set (e.g., \inl{b} in the example) has a default location of the current switch and a default delay of 0. 

When a handler generates events, it places them into a \emph{multi-event header}, represented by the `\emph{b and a}' circle in Figure~\ref{fig:evprog}. The multi-event header contains up to one instance of each event and a counter tracking the number of events generated. 

% Minimum description for a very simple event safety feature that I think is important. 

% Additionally, the multi-event header contains a flag indicating whether the generating handler is an entry handler. The serialized events are put into either a high or low priority queue depending on whether they were generated by an entry handler (i.e., based on \inl{from_entry_handler}). This prevents poorly designed entry handlers, which may invoked by data plane packets at high rates, from disrupting other handlers. 

% Mention "main", or at least kicking off events from controller at startup, in overview by entry and exit events section.

Each time \inl{a} generates an event it populates the respective fields in the multi-event struct and increments the generate counter. 
% and sets the from entry handler flag to false. 

\subsubsection{Event Serialization}
After the ingress pipeline finishes, \lang's serializer writes each event into its own packet, which is then recirculated for further processing. In Figure~\ref{fig:evtrace}, the serializer emits two event packets to switch 1's recirculation port: one carrying event \inl{b} and one carrying event \inl{c}.

The serializer has four components: (1) an \emph{ingress deparser} that encodes the multi-event struct in an outer Ethernet header placed before the packet's Ethernet frame; (2) a \emph{multicast engine configuration} that use the event counter to create one copy of the packet for each event; (3) a \emph{egress parser} that extracts the multi-event fields from a packet; and (4) an \emph{egress serialization table} that converts each clone into a \emph{serialized event packet} that carries at most one event. This table also removes all events from packets that were not created by the \lang multicast groups. 

\subsubsection{Event Dispatching}
% Here, might want to mention that events are given high priority at the ingress parser, so they don't drop. 
When any serialized event packet enters a switch, it is parsed by \lang-generated parsers and passed to an \emph{event dispatcher} in the ingress match-action pipeline. The dispatcher checks the event's \emph{location} and \emph{delay} to figure out how to process it. There are three options.

\heading{Non-local events.} If the event's location is not the current switch, the dispatcher calls a user configured forwarding table to select an output port or multicast group, for events with singleton or group locations, respectively. In the example program, the dispatcher at switch 1 does this for the event packet containing \inl{c}.

\heading{Delayed local events.} For events that are destined to the local switch, but with a delay $> 0$, the dispatcher calls the Event Manager's \emph{delay} function. In the example, this happens to event \inl{c} when it first enters switch 2. 

\heading{Processable events.} An event is ready to be processed when its location is the current switch, and its delay is $0$. At this point, the event leaves the event management layer as the dispatcher passes it to the event handlers. In the example program, the dispatcher at switch 1 recognizes that event \inl{b} is ready to be processed as soon as it arrives, while the dispatcher at switch 2 recognizes that event \inl{c} is ready to be processed after it passes through the delay queue once. 

\subsubsection{Implementing Delay}
The most sophisticated part of the event management layer is the delay function. A simple design would be to buffer the event in a register array along with the time at which it should be executed. By scanning the array periodically, we could find events that were ready to execute. 

This approach is not ideal because it consumes a potentially large amount of register arrays and stateful units in a switch, especially for events with many parameters. An alternate simple approach is to just recirculate the event repeatedly until it is ready. This saves register arrays, but wastes recirculation bandwidth. 

In \lang, we leverage \emph{pausable egress queues} to delay events without wasting register arrays \emph{or} recirculation bandwidth. When the pipeline sees an event that must be handled at the local switch, but at a future time, it places the event in a special ``delay queue'' of the recirculation port. The delay queue is paused most of the time, i.e., it does not emit packets. The delay queue unpauses at a regular interval, e.g., once every 100us. When each event exits the queue, a table in the egress pipeline subtracts the time spent in the queue from the event's delay. The event  recirculates and re-enters the event dispatcher. If the delay is not yet 0, it will re enter the delay queue for another interval. This approach lets us greatly reduce the amount of recirculation bandwidth required by using only a small amount of packet buffer space and a small, fixed number of non-stateful ALUs in the match-action pipeline.  

\lang times the delay queue using PFC (Priority Flow Control) packets. It configures the switch's packet generator to produce a constant, low-rate stream of PFC packets, e.g., 100,000 PFC packets per second. We achieve unpausing at regular intervals by interleaving two streams. First, a higher rate stream of \emph{pause PFCs} that each instruct the queue to pause for a long period of time. By itself, this stream would keep delayed events buffered indefinitely. However, \lang also configures the packet generator to produce a low rate stream of \emph{unpause PFCs}. When an unpause PFC arrives, the queue opens for a short amount of time and sends events until the next pause PFC arrives. 


\subsection{Integration with Native P4}
Although \lang generates many different components, these components are easy to integrate into a P4. We link \lang-generated code into native P4 with a simple script, but manual linking is also feasible. 

\begin{itemize} 
	\item All of the \lang-generated functions for the Event Manager are placed at the beginning of their respective units (e.g., parser, deparser, ingress match-action) and called unconditionally. The functions themselves determine if they must do anything. 
	\item The event handling block is placed at a fixed point in the ingress match-action pipeline program that crosses all control paths. In our linking script, programmers use the \inl{@^dispatch^} pragma to specify where it should be placed, as described in \ref{sssec:p4mainterface}. 
	\item \lang uses a small number of multicast groups, queues, and packet generator program slots. It leaves ample of these resources free for a native P4 program. Assuming the program does not attempt to use resource instances that \lang has reserved, no integration is necessary.
\end{itemize}	


% \begin{figure*}[t]
% \begin{center}
% 	\includegraphics[width=\linewidth]{figures/ingresspipe.pdf}
% 	\caption{Ingress pipeline layout of P4 / \lang program. Shaded boxes are \lang-compiler generated.}
% 	\label{fig:ingresspipe}
% \end{center}
% \vspace{1em}
% \begin{center}
% 	\includegraphics[width=\linewidth]{figures/egresspipe.pdf}
% 	\caption{Egress pipeline of a P4 / \lang program. Shaded boxes are \lang-compiler generated.}
% 	\label{fig:egresspipe}
% \end{center}
% \end{figure*}

% The \lang linker takes compiler generated objects (handlers, event defs, parsers, deparsers, multicast engine configurations, etc.) and a lightly annotated P4 program. Based on the annotations, it inlines the \lang-code into the P4 program to produce a pipeline in the form of~\ref{fig:ingresspipe} and~\ref{fig:egresspipe}.


% 

==> sections/old/compiler_old.tex <==
\section{The DPT Compiler}
Reiterate goal: compile DPT code into target-specific P4 that is efficient, in terms of pipeline resource utilization, and can compile without requiring manually added pragmas. 

Show compiler overview diagram. Generates several components: parse tree extensions (to parse events); pipeline of match-action tables (handlers); deparsers (event generation); event queues (to submit local and remote events). 
The most important (and interesting) topic is compiling event handlers to match action tables. Second most important is how we implement event queues.

\subsection{Event Handlers}
Goal: leverage the switch's TCAM to eliminate control flow dependencies, transforming a "tall and narrow" program (do a few ops, branch, do a few more) into an equivalent "short and flat" program (do as many ops as possible in each stage). Ultimately, we want to fit as many instructions into each action as possible, as many actions into each table as possible, and as many tables into each stage as possible. 

Approach: 
\begin{itemize}
\item Convert DPT into an IR where every statement has a predicate that check the exact conditions that must be true for the statement to execute. 
\item re-organize the program into a dataflow graph of these guarded statements. 
\item apply a greedy instruction selection algorithm to merge guarded statements together into tables and place tables in stages. 
\end{itemize}

\makeunderscoreactive
\begin{figure}[t]
\footnotesize
\noindent\rule{\columnwidth}{.1em}
\setlength{\grammarparsep}{7pt plus 1pt minus 1pt}
\begin{grammar}
<guarded_cmd> ::= <guard> -> <guarded_list>

<guard> ::= <boolean_exp>

<guarded_list> ::= `[' <operation> \{`;' <operation>\} `]'

<guarded_cmd_set> ::= `{' <guarded_cmd> \{`,' <guarded_cmd>\} `}'

<alternative> ::= `if' <guarded_cmd_set> `fi'

<program> ::= <alternative> \{`;' <alternative>\}

\end{grammar}
\vspace{-0.5em}
\noindent\rule{\columnwidth}{.1em}%
\vspace{4pt}
\caption{The DPT intermediate representation.}
\label{fig:irgrammar}
\end{figure}
\makeunderscoreletter

\subsubsection{Intermediate Representation}
Figure~\ref{fig:irgrammar} shows the intermediate representation of DPT programs, based on Guarded Command Language~\cite{dijkstra1975guarded}. In this representation, a program is a list of \textit{alternative} statements. Each alternative executes the guarded list of one guarded command whose guard evaluates to true. A guarded list contains instruction-level operations that execute in parallel.

Figure X illustrates the algorithm used to transform DPT into DPT-IR. 

\subsubsection{Optimization Passes}
The compiler derives a dataflow dependency graph from alternative statements in the IR. Using this dependency graph, it applies a greedy instruction selection algorithm to map alternative statements to a layout of P4 
tables. 

Figure X illustrates the algorithm. The compiler iterates over all tables in a pipeline with a fixed width 
(i.e., number of tables per stage) and unbounded length (i.e., number of stages), maintaining a list 
of unplaced alternative statements. For each table, the algorithm attempts to place each unplaced alternative statement in the table, subject to the constraints in Table Y. 

\subsubsection{P4 Code Generation}
Using the layout plan, the DPT compiler generates straightline P4 code, i.e., the \textit{apply} statement of its 
\textit{control} block consists of only a sequence of table applications. The tables are annotated with pragmas that specify 1) the earliest stage that the DPT compiler believes each table can be placed in; and 2) which tables have data dependencies. The stage annotations serve as a hint to the Tofino compiler that allow it to find better layouts and compile faster, while the data dependency annotations ensure that even when the compiler must place tables later in the pipeline (due to lower level constraint that the DPT compiler does not consider), the program will remain functionally correct.

\subsection{Event Generation and Queuing}
Local and remote event queues. 


\subsection{Implementation}
XXX lines of OCAML. P4-tofino backend and linker. Backend generates P4 code. Linker replaces DPT extern calls with inlined DPT code and hard codes switch identifiers. 

\subsubsection{Integration}
\begin{figure}[!t]
	\begin{lstlisting}[style=P4Block]
	#include "dpt_generated.h"
	control !Ingress!(inout header_t hdr, inout metadata_t md) {
		!DptDispatcher!() dpt;
		action !set_dst!(addr) { 
			md.dpt.eventType = IP_IN;
			md.dpt.dpt_ip_in.dst = addr; 
		}
		table !setPacketId! {
			key = {ip.dst : exact;}
			actions = {set_ip; noop;}
			const default_action = noop;
		}
		apply {
			setPacketId.apply();
			dpt.apply(md.dpt);
			if (md.dpt.eventType == IP_OUT)	{
				md.ucast_egress_port =  md.dpt.dpt_ip_out.egrPort;
			}
		}
	}
	\end{lstlisting}
	\caption{Calling DPT from P4 ingress.}
	\label{fig:p4call}
\end{figure}

A \lang program gets called at a fixed point in the ingress block of a lower level P4 program. For example, Figure~\ref{fig:p4call} shows how the \exprog is used. The \lang compiler generates the \code{DptDispatcher} control block, which contains all the event declarations and handlers for the \exprog. In the P4 ingress block, the \code{setPacketId} table generates a packet entry event by populating the \code{dpt.eventType} and \code{md.dpt.dpt_ip_in} fields. It calls the \code{DptDispatcher} and, if the dispatcher returned a \code{ip_out} packet exit event, sets the packet's egress port accordingly. 

\reminder{Missing: auto generated parser and deparser. Composing inlined and background DPT handlers.}


% Events can be generated by the underlying P4 program, an event handler running on the local switch, or an event handler running on a remote switch. 



% Enter DPT programs from P4, by calling an extern function. Return to P4 programs by generating a continue event. 

\subsubsection{Development}
DPT has two backends: main backend that emits P4\_16-Tofino; development backend that emits Python which runs in a custom-built software switch and containerized virtual network environment (similar to Mininet.. Just call it Mininet?)

==> sections/old/implicitrestrictions.tex <==
\section{PISA ALU Constraints}
\label{sec:syntax}

PISA programmers must typically ensure that their code fits the capabilities of the individual ALUs of the pipeline. This is difficult in simple packet processing, and quickly becomes daunting for more complex applications that integrate control processes. 
%
This section describes the two mechanisms that \lang introduces to free developers from this burden.


\subsection{Constraining Stateful Operations}
\label{ssec:memops}
The primary goal of most control tasks, regardless of where they run, is to update and maintain the state used to handle data packets. This makes stateful operations critical in data-plane applications with integrated control.

However, stateful operations are challenging to write. The core problem is not necessarily that the underlying stateful ALUs have limitations, but rather that their nuanced constraints are left \emph{implicit} in today's data-plane languages. For example, in P4, programmers write \code{RegisterActions} with arbitrary blocks of C-like code to process a single register access. Unsurprisingly, it is easy to write a \code{RegisterAction} that cannot compile, but difficult to figure out why. The ``decision'' that a particular register action is too complex is made in part of a compiler's back-end that is far removed from the source code. When compilation fails, programmers have no direct way of figuring out what went wrong. For example, here is a register action that does not compile: 
\begin{lstlisting}[style=P4Snip]
void apply(inout bit<32> memCell, out bit<32> retCell) {
    if (memCell > hdr.ip.src_addr) { retCell=memCell; }
    else { retCell=hdr.ip.src_addr;}
}
\end{lstlisting}

After some trial and error (including the message \code{error: RegisterAction too complex}), we can finally get this to compile by rewriting it as: 
\begin{lstlisting}[style=P4Snip]
void apply(inout bit<32> memCell, out bit<32> retCell) {
    bit<32> tmp;
    if (memCell <= hdr.ip.src_addr) {tmp=hdr.ip.src_addr; }
    else {tmp=memCell;}
    retCell = tmp;
}
\end{lstlisting}

% The compiler's error tells us that the output variable \code{retCell} must be set by the same variable in all code paths. We might try resolve the issue with a temporary variable.

% \begin{lstlisting}[style=P4Snip]
% void apply(inout bit<32> memCell, out bit<32> retCell) {
%     bit<32> tmp;
%     if (memCell > hdr.ip.src_addr) { tmp=memCell; }
%     else { tmp=hdr.ip.src_addr;}
%     retCell = tmp;
% }
% \end{lstlisting}

% Now, the compiler simply tells us \code{error: RegisterAction too complex}. Is this because of the newly added temporary variable? No. In fact, the register action is \emph{not} too complex. By reversing the branches we can finally get the operation to compile. But the only way to figure this out is through trial and error. 
% \begin{lstlisting}[style=P4Snip]
%     if (memCell <= hdr.ip.src_addr) {tmp=hdr.ip.src_addr; }
%     else {tmp=memCell;}
% \end{lstlisting}

\heading{MemOps.} 
\lang avoids scenarios like the one above by making restrictions on stateful operations \emph{explicit and obvious} to the programmer. 
We do this by providing a \emph{syntactic} description of what these operations must look like. We call these \emph{memops}, and each is a function of two arguments whose body consists of either a single return statement or a single if statement containing one return statement in each half. Furthermore, each variable may be used at most once in each expression, and only certain binary operators are allowed. When a user declares a memop, we automatically check that its body satisfies these requirements. If this check passes, the programmer is guaranteed that the operation will compile; if not, our compiler can explain exactly what is wrong. 

For example, the stateful operation from above would be:
\begin{lstlisting}[style=SmallDptBlock]
memop get_max(int stored, int addr) {
	if (stored > addr) { return stored; }
	else { return addr; }
}
...
int cur_max = Array.getm(max_arr, myidx, get_max, src_addr);
\end{lstlisting}
% \dl{Pretty sure this memop is actually get_min}
A memop is then used by passing it to Array method calls throughout the program, as shown above for \code{get_max}. The \lang compiler translates each call that uses a memop into a P4 register action that compiles to the Tofino. The restricted syntax of memops means that they have only a finite number of possible forms, making it easy to verify that all of them do in fact compile.



%We can guarantee that any syntactically correct {memop} translates to a Tofino-compatible register action because there are a small, finite number of possible {memops}---$68$, to be exact, not counting different types of binary and arithmetic operations, or multiple constant variables that can be folded at compile time. A register action uses at most two {memops}, one that returns to a metadata variable and a second that returns to the element of the register array. Thus, the \lang compiler can produce up to $4624$ different forms of a register action, all of which compile to the Tofino. 


\subsection{Simplifying Stateless Operations}

Operations over non-persistent variables (i.e., variables stored in packet headers or metadata) also face constraints based on the capabilities of individual ALUs. 
%For example, expressions that are too complex for a single ALU will cause program compilation to fail.
In practice, programmers can often avoid issues with careful programming discipline. For example, on the Tofino: 

\begin{enumerate}[leftmargin=*] 
\item Break down each operation over packet metadata into a sequence of simple operations, where a ``simple operation'' is an expression that maps directly to a single Tofino ALU instruction. 

\item Encapsulate each ``simple operation'' in its own action and table, to ensure that no passes in the P4 compiler fold multiple simple operations together. 
\end{enumerate}

This will produce a program that does not violate ALU-level constraints, but is extremely tedious for programmers. 


\lang's compiler eliminates this burden by automatically translating every statement in a \lang handler into a \emph{sequence of single-action P4 tables}. Every single-action P4 table is simple enough to use at most \emph{one} ALU or stateful ALU, and thus can always compile to a PISA switch. There are three main types of single-action tables.

% that data plane developers must often track. For example, this simple P4 snippet will not compile to the Tofino: 
% \begin{lstlisting}[style=P4Snip]
%   bit<32> lastPingedTs = getLastPinged.execute(egrPort);
%   if (md.ts - lastPingTs > TIMEOUE_THRESH)
%   	egrPort = NO_ROUTE;
% \end{lstlisting} 

% The 

% This code snippet does not compile on the Tofino because the left-hand side of \inl{if} condition is a compound operation that cannot be fit into any one of the Tofino's Comparison units. To fix this, a programmer might try to split the operation into two lines.
% \begin{lstlisting}[style=P4Snip]
%   bit<32> delta = md.ts - lastPingTs;
%   if (delta > TIMEOUT_THRESH) ...
% \end{lstlisting}
% This would also fail to compile. In the P4 front-end, an optimizing pass that is oblivious to the limitations of the Tofino will inline the right hand side of \inl{bit<32> delta = md.ts - lastPingTs;} into subsequent code, silently undoing the attempt to simplify operations. The fix is to encapsulate the statement in an action and call that action in the apply block.

% Unfortunately, the compilation would still fail because of a second hardware limitation that is not represented in P4: the Tofino can only support less/greater than comparisons for variables smaller than 12 bits. The most general workaround, in this case, is using a saturating subtract operation (i.e., one that cannot underflow) to transform the \inl{>} test into a \inl{!=} test. 

% \heading{Serializing operations.} 
% The above example demonstrates an important principle: operations over non-persistent variables can always be broken up into multiple steps. \lang's compiler leverages this principle, and the guarantees that memops provide, to translate all the \lang handlers in a program into a P4 program that can never violate ALU-level constraints. 


% The idea is to transform every statement in a \lang handler into a \emph{sequence of single-action P4 tables}. Every single-action P4 table is simple enough to use at most \emph{one} ALU or stateful ALU, and thus can always compile to a PISA switch. There are three main types of single-action tables.

\subheading{Operation table} An operation table uses a single ALU to evaluate a binary expression over two local variables and assign its result to a third local variable. For example, \\\inl{idx = idx + NUM_PORTS;} translates to: 
\begin{lstlisting}[style=SmallP4Snip]
action do_idx_add {idx = idx + NUM_PORTS;}
table tbl_idx_add { actions = {do_idx_eq;}
	const default_action = {do_idx_eq;} }
\end{lstlisting}
% An operation table is guaranteed to not violate ALU constraints because it only accesses at most three P4 metadata fields and is restricted to operations that the ALUs can support. 

\subheading{Memory operation table} A memory operation table uses a single stateful ALU to update one element in a P4 register array. It is a direct translation of a call in \lang to an Array method that is passed a memop. For example, \\\inl{Array.setm(tcp_cts, port, plus, 1);} translates to:
\begin{lstlisting}[style=SmallP4Snip]
RegisterAction<bit<32>,bit<32>,bit<32>>
  (tcp_cts) setm_1 = {
  void apply(inout bit<32> mem, out bit<32> ret) {
    mem = mem + 1;
  } };
action do_setm_1() { setm_1.execute(port);}
table tbl_setm_1 { actions = {do_setm_1; }
    const default_action = {do_setm_1;} }
\end{lstlisting}
% A memory operation table is guaranteed to not violate stateful ALU constraints because of the syntactic restrictions on memops.


\subheading{Branch table} A branch table uses the table itself to compare a local variable to a constant. It calls either a true or false action. These actions determine which execution path a program takes in the subsequent stages of a PISA pipeline. For example, \inl{if(proto != TCP)} translates to:
\begin{lstlisting}[style=SmallP4Snip]
action if_true(); action if_false();
table tbl_if {	
	keys = {proto : ternary;}
	actions = {if_true; if_false;}
	entries = {
		(TCP) : if_false;
		(_)   : if_true;
}	}
\end{lstlisting}
% A branch table is guaranteed not to violate constraints of what can be matched in a single table because it only ever tests one P4 metadata field against a constant. 

Since each single-action table maps directly to a primitive in the PISA pipeline, a \lang program represented as a sequence of such tables will \emph{never violate ALU-level constraints}. 

% A \lang program represented as a sequence of single-operation P4 tables is straightforward to compile into a block of P4 -- we use \inl{apply()} to call each of the operation tables and \inl{switch()} on each branch table. 

% By construction, a \lang program represented as a sequence of single-operation tables will \emph{never violate ALU-level constraints}. 


% The drawback, however, is that breaking down operations into multiple sequential steps produces an overall block of P4 code that can require many stages. As the next section describes, the compiler's backend makes up for this by optimizing the code. 

% \lang's general solution to eliminating the implicit restrictions on all non-stateful operations (including branching operations) is to reduce every statement into a sequence of primitive statements that can each be implemented in a single Tofino-compatible P4 table \jrex{confusing. how can a single table implement a "sequence" -- don't sequences of operations require multiple pipeline stages? I'm getting a bit confused.}. If the above snippet was from a \lang program, the front-end of the \lang compiler would automatically perform the sequence of transformations that we described above.

% This has the unavoidable drawback of increasing the code's critical path length, which can stop a program from fitting in a PISA pipeline with limited stages. However, as Section~\ref{ssec:p4optimizations} describes, \lang's back-end compensates for this by optimizing the program to find and exploit fine-grained instruction-level parallelism, which significantly reduces the critical path length of complex programs. \jrex{sounds intriguing but I don't understand how. and then the subsection ends with a backwards pointer.}




\subsection{Minimizing Number of Pipeline Stages}
\label{ssec:p4optimizations}
\begin{figure}[t]
% \includegraphics[width=.3\linewidth]{figures/seqgraph.pdf}
\begin{lstlisting}[style=SmallDptBlock]
Array nexthops = new Array<<32>>(NUM_HOSTS);
Array pcts = new Array<<32>>(NUM_PORTS_X3);
Array hcts = new Array<<32>>(NUM_HOSTS);
memop plus(int cur, int x){return cur + x;}

event count_pkt(int dst, int proto);
handle count_pkt (int dst, int proto) {
	int idx = Array.get(nexthops, dst);
	if (proto != TCP) {
		if (proto == UDP)
			idx = idx + NUM_PORTS;
		else 
			idx = idx + NUM_PORTS_X2;
	}
	Array.set(pcts, idx, plus, 1);		
	if (proto == TCP)
		Array.set(hcts, dst, plus, 1);
}
\end{lstlisting}
\includegraphics[width=\linewidth]{figures/controltodataflow2.pdf}
\caption {Optimizations of the P4 representation of a \lang handler. 
The single-action table representation (on the left) requires seven pipeline stages. By inlining conditional tests to eliminate tables dedicated to branching (top right) and then reordering tables according to their data dependencies (bottom right), the \lang compiler reduces this to four pipeline stages.}
\label{fig:cttblgraph} 
\end{figure}


By transforming a \lang program into a sequence of single-action tables, we produce P4 code that may span many pipeline stages. To address this issue, the \lang compiler applies two optimizations that greatly reduce the number of stages required by the resulting P4 code.  
% We describe these optimizations based on the example \lang program in Figure~\ref{fig:cttblgraph}.


% The \lang compiler translates handlers to P4 in three main phases. First, a front-end performs several standard passes, operating on the source language, i.e., function inlining, variable renaming, and subexpression elimination. The output of the front-end is a \lang program composed of \emph{primitive \lang statements} that each only perform a single operation. \jrex{i started getting lost here.  what are these statements? are we still talking about event primitives or something else?} The top of Figure~\ref{fig:cttblgraph} shows a program already in this form. The back-end translates this into a graph of \emph{single operation P4 tables}, like the one shown in Figure~\ref{fig:cttblgraph}(1), using a simple template-based algorithm described in  Appendix~\ref{app:backendfirstpass}.

% The most interesting parts of the compilation process are the optimization phases that follow, which we describe below. The main insight is that P4 compilers only optimize at the coarse granularity of individual tables. This is by design---they do not want to change the semantics of the program. However, this also limits the amount of instruction-level parallelism that the compiler can find. Thus, the \lang compiler focuses on finer-grained optimizations \emph{within} and \emph{across} tables and actions to find more parallelism.

% \heading{Exploiting instruction level parallelism.}
% The templates above give us a way to translate each \lang statement into a single operation P4 table that will compile on the Tofino. However, if the compiler simply emitted these tables, the resulting code would compile to very inefficient P4 code. 

% The main insight is that P4 compilers only perform operations at the coarse granularity of individual tables. By design, they do not change the structure or contents of tables or actions. This limits the amount of instruction level parallelism that the compiler can find. Thus, the \lang compiler focuses on finer-grained optimizations \emph{within} and \emph{across} tables and actions to find more parallelism.

\heading{Inlining branch operations.}
Branching on a table is expensive in a PISA switch because the tables that come next in the program must be placed in a subsequent stage. 
For example, in the following P4 code, \inl{tbl_B} and \inl{tbl_C} must be placed in a stage after \inl{tbl_A}. 
\begin{lstlisting}[style=SmallP4Snip]
switch(tbl_A.action_run()) {
    if_true :  {tbl_B.apply(); }
    if_false : {tbl_C.apply(); } }
\end{lstlisting}

This makes the single-action table representation of a \lang handler require many stages because of its \emph{branch tables}. For example, Figure~\ref{fig:cttblgraph}(1) shows this representation of a simple \lang handler. It requires seven pipeline stages to execute, three of which are used by branch tables. 

The \lang compiler eliminates the need for branch tables by 
transforming the operation tables (i.e., the tables that do not branch) so that each table checks all the conditions necessary for its own execution, using static match-action rules. If the conditions are met, the table executes its single action. If the conditions are not met, the table executes a no-op. 
%
For example, consider the table \inl{idx_eq_0}. By following the control path from the root node to the table in Figure~\ref{fig:cttblgraph}\textbf{(1)}, we see that it only executes when \inl{(proto != TCP) && (proto != UDP)}. Thus, in Figure~\ref{fig:cttblgraph}\textbf{(2)}, the \inl{idx_eq_0} table only executes its action when these conditions are true. 



% \heading{Eliminating control dependencies.}
% The first optimization is to eliminate control flow dependencies between tables. A control flow dependency simply means that if table A is called before table B, it will be executed before table B. Control flow dependencies are expensive in PISA switches because when we branch using a table, the subsequent table must be placed in the next stage. 

% % of branch operations. Consider the following example: 
% \begin{lstlisting}[style=SmallP4Snip]
% switch(tbl_A.action_run()) {
%     if_true :  {tbl_B.apply(); }
%     if_false : {tbl_C.apply(); } }
% \end{lstlisting}



% The first optimization is to eliminate control flow dependencies \jrex{will readers know what these are yet?  a little confusing based on what has been said so far.} by exploiting TCAM. Figure~\ref{fig:cttblgraph}{(1)} shows a control graph for the \inl{count_pkt} handler. In the Tofino, these tables take seven physical stages to execute because of all their control flow dependencies. 

% The \lang compiler eliminates the dependencies by transforming each single operation table so that it checks all the conditions necessary for its own execution. For example, consider the table \inl{idx_eq_0}. By following the control path from the root node to the table in Figure~\ref{fig:cttblgraph}\textbf{(1)}, we see that it only executes when \inl{(proto != TCP) && (proto != UDP)}. Thus, we transform the table so that it executes a no-op unless these conditions are met. 
% % \begin{lstlisting}[style=P4Snip]
% % action do_idx_eq_0 {idx = idx + NUM_PORTS;}
% % table idx_eq_0 {	
% % 	actions = {do_idx_eq_0;}
% % 	keys = {proto : ternary;}
% % 	entries : { // these entries are ordered.
% % 		(TCP) : do_noop;
% % 		(UDP) : do_noop;
% % 		( _ ) : do_idx_eq_0;
% % }	}
% % \end{lstlisting} 

\heading{Merging tables and actions.}
The \lang compiler rearranges tables to further reduce the number of stages used by a program. For example, in Figure~\ref{fig:cttblgraph}(2), the table that implements \inl{Array.set(hcts, dst, plus, 1);} (\inl{hcts_fset}) does not \emph{actually} need to execute last. It does not have any data flow dependencies on previous tables. That is, its execution condition and input variables are not modified by any other tables in the program, so it can be executed in parallel with the first table, as shown in Figure~\ref{fig:cttblgraph}(3). 

Ultimately, the only factors that matter for determining the layout of tables are data flow dependencies and the resources (tables, ALUs, etc) in each stage.
%-- i.e. a PISA switch only has a limited number of tables, ALUs, etc, in each stage. 
Tables themselves are a primary bottleneck---there are typically far more ALUs than tables in a PISA stage. 

\begin{figure}[t]
\includegraphics[width=.9\linewidth]{figures/tblmrg.pdf}
\caption {Merged tables for the program in Figure~\ref{fig:cttblgraph}.}
\label{fig:mergedtbls} 
\end{figure}


This motivates \lang's second main optimization: it merges all the single-action tables into a layout of multiple-operation tables according to data dependencies. This is possible because \lang-generated tables use only static rules. Figure~\ref{fig:mergedtbls} shows how tables from the example in Figure~\ref{fig:cttblgraph} get merged. 

The algorithm is a simple greedy instruction selection. It  takes a list of single operation tables to place and two parameters, $M$ and $N$, that define the number of stages in the pipeline and the number of tables per stage. For each single operation table $t$, it iterates over all $M$$\cdot$$N$ tables to find the earliest multi-operation table that $t$ can be merged into. This decision is based on data flow constraints, a simple model of the free resources in each stage, and a small number of platform-specific constraints.
%, e.g., for the Tofino, we require that all operations that access the same register array map to the same multi-operation table. 

When the algorithm finds a multi-operation table that $t$ can be merged into, it generates a new table that is the cross product of the two. This new table replaces the multi-operation table in the pipeline. Placement ends when either all single operation tables have been merged, or the algorithm reaches a single operation table that cannot be placed. 


% Eliminating control flow gives us more opportunities to execute tables in parallel. However, each table still only implements one primitive \lang statement. This is inefficient because each stage of the pipeline has many more ALUs than it does tables. In more complex programs the number of tables required will force us to spill into a subsequent stage before we can use all of its ALUs. 

% \begin{figure}[t]
% % \includegraphics[width=.3\linewidth]{figures/seqgraph.pdf}
% \includegraphics[width=\linewidth]{figures/table_merging_example_pdf.pdf}
% \caption {Merged tables for the program in Figure~\ref{fig:ctprog}.}
% \label{fig:mergedtbls} 
% \end{figure}


% The penultimate phase of the \lang compiler reduces the number of tables by combining the single operation tables into a layout with a fixed number of multiple operation tables. Figure~\ref{fig:mergedtbls} shows how the tables in the example get laid out. 

% The algorithm is a simple greedy instruction selection. It  takes a list of single operation tables to place and two parameters, $M$ and $N$, that define the number of stages in the pipline and the number of tables per stage. For each single operation table, it iterates over all $M$$\cdot$$N$ tables to find the earliest pipeline table that it can merge into, subject to data flow constraints and a simple model of the remaining free resources in a stage. 

% When the algorithm finds a table that can fit the current single operation table, it generates a new merged table that is the cross product of the two. This new table replaces the merged table in the pipeline. Placement ends when either all single operation tables have been merged, or the algorithm reaches a single operation table that cannot be placed. 

% \heading{Emitting P4.}
% The last phase of the compiler annotates merged tables with Tofino-specific pragmas to help the P4 compiler find a layout that uses fewer stages. The most important pragma is \emph{ignore_dependencies}, which indicates control flow dependencies that can be ignored. The \lang compiler uses this to inform the P4 compiler that a table only depends on the ones that come before it in the data flow graph. 

% Finally, after generating the pragmas, the \lang compiler emits a block of P4 code that contains the merged tables, all the objects that they use, and a block of table call statements. 

% \heading{Integration with native P4.}
% \lang links generated artifacts into a host program with a simple preprocessing script. The event management library functions are always called at the beginning of their respective units (e.g., parser, deparser, ingress match-action). The event handling block is placed at a fixed point in the ingress match-action pipeline program that crosses all control paths. P4 developers use a simple \inl{@^dispatch^} pragma to specify where it should be placed. 
% % The functions themselves determine if they must do anything. 




% \lang uses a small number of multicast groups, queues, and packet generator program slots. Assuming the program does not attempt to use resource instances that \lang has reserved, no integration is necessary.



% The core problem is that the underlying P4 compiler only optimizes at the coarse granularity of \emph{tables}. By design, it does not modify the content of the tables or actions. This limits the amount of parallelism that we can exploit, because there are far fewer tables in each stage than there are ALUs or TCAM entries. 

% To improve parallelism, the 

% However, if we used these tables directly in a P4 control block, we would end up with a P4 program that used the Tofino's highly-parallel architecture very inefficiently. 





% In applications with multiple handlers, this table is placed at the root of the table control graph. 


% \subsection{Integration with Native P4}
% Although \lang generates many different components, these components are easy to integrate into a P4. We link \lang-generated code into native P4 with a simple script, but manual linking is also feasible. 

% \begin{itemize} 
% 	\item All of the \lang-generated functions for the Event Manager are placed at the beginning of their respective units (e.g., parser, deparser, ingress match-action) and called unconditionally. The functions themselves determine if they must do anything. 
% 	\item The event handling block is placed at a fixed point in the ingress match-action pipeline program that crosses all control paths. In our linking script, programmers use the \inl{@^dispatch^} pragma to specify where it should be placed, as described in \ref{sssec:p4mainterface}. 
% 	\item \lang uses a small number of multicast groups, queues, and packet generator program slots. It leaves ample of these resources free for a native P4 program. Assuming the program does not attempt to use resource instances that \lang has reserved, no integration is necessary.
% \end{itemize}	




% \begin{figure}[t]
% \small
% \setlength{\interspacetitleruled}{0pt}%
% \setlength{\algotitleheightrule}{0pt}%
% \removelatexerror
% \begin{algorithm}[H]
% \setstretch{.95}
% \DontPrintSemicolon


% \textcolor{gray}{/* {\footnotesize Global state.}*/}\;


% \textcolor{gray}{/* {\footnotesize Main placement algorithm.}*/}\;
% \SetKwProg{Fn}{Function}{}{}
% \Fn{placePrimitiveTables(primitiveTables):}{
% 	$\textit{unplaced} \gets \textit{primitiveTables}$\;
% 	\For{{\bf each} stage {\bf in} stages} {
% 		\For{{\bf each} table {\bf in} tables} {
% 			$\textit{stillUnplaced} \gets \textit{[]}$\;
% 			\For{{\bf each} primitive {\bf in} unplaced} {
% 	    	    \uIf{canPlace(primative, stage, table);}{

% 	    	    }
% 	    	    \Else{
% 			        $\textit{stillUnplaced.append(primitive)}$\;
% 			    }
% 			}
% 			$\textit{unplaced} \gets \textit{stillUnplaced}$\;

% 		}
% 	}	
% }
% \SetKwProg{Fn}{Function}{}{}
% \Fn{canPlace(primitiveTable, stage, table):}{


% }



% \end{algorithm}
% \caption{Pipeline layout algorithm.\reminder{Todo: finish writing up the algo.}}
% \label{fig:layoutalgo}
% \end{figure}


% % \section{Resolving Implicit Restrictions}
% \jrex{the next few paragraphs are pretty abstract.  should we focus more specifically on \emph{action} processing? how does this relate to putting control in the data plane, specifically?}
% One of the most challenging aspects of programming the data plane is dealing with implicit restrictions \jrex{restrictions on what?}. Data-plane languages, like P4, have general syntax designed for a wide range of different architectures (e.g., NPUs, PISA pipelines, FPGAs.) The assumption, from the language perspective, is that target-specific back-ends will take care of low-level translation details.

% Unfortunately, this is not so easy. Inherent architectural restrictions, or the desire to conform to a rigid cost model (e.g., one statement always executes in one ALU) can make it impossible to compile parts of a program to a specific target. Ultimately, back-ends are written with the \emph{reverse} assumption---that the front-end will only give it programs that can map to the underlying hardware. This disconnect makes it hard to figure out what will and will not compile in a language and frustrates efforts to work around limitations. 

% This section introduces \lang's solutions to resolve two general classes of implicit restrictions that have a significant impact on applications with integrated control: branching and stateful operations. \jrex{why these two? are these the main two things that matter? what is the scope of "implicit assumptions" that the reader should be worrying about, and why?}

% \lang solves this issue with two mechanisms: expression simplification, for stateless operations, and syntactically restricted memory operations, for stateful operations. 

% \subsection{Branching Restrictions}
% % P4's \code{if/else} statements have a specific semantic meaning in a PISA pipeline. They map to  \emph{gateway tables}, small dedicated TCAMs at the beginning of each stage. This is an optimization that lets P4 programs perform a branch operation without increasing its number of stages.

% Control operations often have complex decision logic~\cite{maple}. Branches, e.g., \code{if/else} statements, are the cornerstone of such operations, and these operations have many implicit restrictions in today's languages. For example, in P4, consider the following syntactically valid code: 
% \begin{lstlisting}[style=P4Snip]
%   bit<32> lastPingedTs = getLastPinged.execute(egrPort);
%   if (md.ts - lastPingTs > TIMEOUE_THRESH)
%   	egrPort = NO_ROUTE;
% \end{lstlisting} 

% This code snippet does not compile on the Tofino because the left-hand side of \inl{if} condition is a compound operation that cannot be fit into any one of the Tofino's ALUs. To fix this, a programmer might try to split the operation into two lines.
% \begin{lstlisting}[style=P4Snip]
%   bit<32> delta = md.ts - lastPingTs;
%   if (delta > TIMEOUT_THRESH) ...
% \end{lstlisting}
% This would also fail to compile. In the P4 front-end, an optimizing pass that is oblivious to the limitations of the Tofino will inline the right hand side of \inl{bit<32> delta = md.ts - lastPingTs;} into subsequent code, silently undoing the attempt to simplify operations. The fix is to encapsulate the statement in an action and call that action in the apply block.

% Unfortunately, the compilation would still fail because of a second hardware limitation that is not represented in P4: the Tofino can only support less/greater than comparisons for variables smaller than 12 bits. The most general workaround, in this case, is using a saturating subtract operation (i.e., one that cannot underflow) to transform the \inl{>} test into a \inl{!=} test. 

% \heading{\lang's solution.} 
% \lang's general solution to eliminating the implicit restrictions on all non-stateful operations (including branching operations) is to reduce every statement into a sequence of primitive statements that can each be implemented in a single Tofino-compatible P4 table \jrex{confusing. how can a single table implement a "sequence" -- don't sequences of operations require multiple pipeline stages? I'm getting a bit confused.}. If the above snippet was from a \lang program, the front-end of the \lang compiler would automatically perform the sequence of transformations that we described above.

% This has the unavoidable drawback of increasing the code's critical path length, which can stop a program from fitting in a PISA pipeline with limited stages. However, as Section~\ref{ssec:p4optimizations} describes, \lang's back-end compensates for this by optimizing the program to find and exploit fine-grained instruction-level parallelism, which significantly reduces the critical path length of complex programs. \jrex{sounds intriguing but I don't understand how. and then the subsection ends with a backwards pointer.}



==> sections/old/intro.tex <==
\section{Introduction}

% DPW: switch hardware is useful but complicated/constrained
Linerate programmable switch hardware has enabled a host of new
network applications such in-network telemetry, dynamic 
security monitoring and enforcement, failure detection and recovery, traffic
engineering, and application-level caching.
However, this hardware is also complicated, coming with many specialized
computing components.  For instance, Barefoot's (Intel's?) Tofino chip
contains multiple packet-processing pipelines.  Each pipeline contains a
set of queues as well as a series of compute stages.  The stages themselves
contain ALUs, stateful ALUs, hash units, containers for packet data and meta-data, TCAM tables, and SRAM memories.  Numerous constraints govern
how these units can be used and the way packet data can flow between them.

% DPW: P4 allows you to program the hardware but is low-level/verbose
P4~\cite{p4} protects application developers from some of this complexity
by providing a language for programming this hardware.  The language contains some familiar components such as imperative variables, arrays, conditionals and
sequencing.  These features provide the raw bones for crafting interesting new
applications

but it also provides a variety of domain-specific elements
such as packet parsers and deparsers, tables, and packet-processing actions.
Moreover, some key parts of the system, such as queue management and recirculation,
must still be programmed using device-specific microcode.
The net effect is that P4 remains a very low-level programming language \reminder{in which many applications are hard to express. Concurrent or distributed applications~\cite{hsu2020contra, zhou2019hypertester, starflow} are especially challenging because they require programming many different types of components. For example, ...}
\dpw{John --- Maybe give 1 or 2-sentence example of something that takes many
lines of P4 code and a number of features right here.  eg:  For instance,
to alert a neighboring device of a failure, a P4 programmer must write
a packet parser, program the mirroring engine, interpret the packet, all
of which takes XXX lines of code to implement "send X" and "receive X". 
Probably emphasis verbose.}
\js{Specifically calling out concurrent / distributed tasks here might help tie events in better?}

% DPW: P4 does not hide the hardware constraints
Worse yet, P4 does not encapsulate the many low-level hardware
constraints of an ASIC like the Tofino.  Indeed, programming
for the Tofino is often a frustrating experience because
apparently-valid P4 programs often simply fail to compile. 
These programs might contain an arithmetic expression that is just 
a bit too complicated to be executed by a single Tofino action, \reminder{a sequence of conditional branches that is too long for a single Tofino stage to support, or a pair of independent control flows that access persistent state in an inconsistent order.}
\dpw{John--extend this sentence to give a couple more examples of things that can cause
compilation to fail and that we can actually solve with our technology}. 
\js{Added 2 example, will refine and come up with more.}
Because P4 is intended to be hardware-independent, the language definition
itself does not explain why such failure occur.  Programmers are usually left
to try to infer what is wrong with their program from the low-level
\emph{outputs} of the compiler, such as the number of hardware stages
generated \dpw{John, give better example. Ideally something our system does 
really well.}, rather than being given direction in terms of the source
program they have constructed.


% DPW:  How does other work tackle this?
One way to tackle these problems is to design higher-level languages
for programming switch hardware and to use compiler or program synthesis
technology to generate the low-level code.  Recent research on Chipmunk~\cite{chipmunk}, Domino~\cite{domino}, Lyra~\cite{lyra} and
P4All~\cite{p4all} takes such an approach.  Each of these systems
lifts the level of abstraction at which programmers define their intent
and then uses optimization technology to generate P4- or hardware-level
packet-processing pipelines, which sometimes even span multiple devices. 
When a programmer writes a program that \emph{can be compiled}, these systems
are extremely effective, performing as well or better than hand-tuned
pipelines in terms of metrics like number of pipeline stages used.  In many
cases, they also cut down the lines of code a programmer must write 
dramatically. \reminder{However, these systems do not abstract some of the most difficult 
(and also powerful) components of the Tofino, e.g., recirculation ports or programmable queues, which are critical for many applications.}
\js{To tie events in, the above line tries to mention that current systems lack abstractions for parts of the Tofino that distributed/concurrent applications need.}
Further, when programmers write a program that \emph{cannot be compiled}, something that happens regularly to both
experts and non-experts when navigating the pitfalls of irregular switch hardware, these languages have little to say.  Typically, compilation is
attempted with little feedback about what goes wrong when it fails.


To this paper, we introduce \lang, a new programming
language for Barefoot Tofino.  \lang compliments recent
research on Chipmunk~\cite{chipmunk}, Domino~\cite{domino} and the like,
by introducing a \emph{correct-by-construction} design to the 
field---one that eliminates combinations of features that do not compile
whenever possible.  When a programmer writes a code fragment that lives outside our source-level language definition, we give error messages in terms of the source program, not in terms of the underlying hardware, and we point to locations in the source code that must be fixed, not to underlying hardware resources.

Our new design achieves it goals through the use of three inter-dependent
mechanisms.

\begin{enumerate}
    \item \textbf{Syntactic constraints}: We define domain-specific,
    source-language constraints to characterize \emph{memops}, the 
    \reminder{stateful} operations that can be executed in a single stage of a pipeline.
    Operations that cannot be executed in a single stage are not classified
    as memops.
    \item \textbf{Types and effects}: We develop a novel, ordered type-and-effect system that
    limits the way programs interact with persistent memory.  Since that
    memory must be allocated to a particular stage of a packet-processing
    pipeline, access to the memory in inconsistent order by different
    components of a program make it impossible to compile without
    recirculation (too costly a mechanism to be used on most packets).
    Our ordered type system has been designed to support type inference,
    freeing programmers from the need to use complex type annotations,
    while also providing source-level feedback when programming errors occur.
    \item \textbf{Well-designed primitive abstractions}:  We develop
    abstractions for the use of stateful memory such as arrays and
    registers designed to be correct-by-construction.  These abstractions
    may be accessed via interfaces that exploit our domain-specific 
    type system and syntactic constraints.
\end{enumerate}

On top of its correct-by-construction design, 
\lang layers an event-driven
programming framework inspired, in part, by Reppy's Concurrent ML~\cite{concurrentml}. In this framework, programmers may declare
new event types that carry data from one place or time to another.
Event handlers recognize and process events and may in turn generate
new events that can materialize here and now, on the current device, or elsewhere and later, as directed, on other \lang devices in the network. 
\js{Do we want to mention that these features/framework abstracts Tofino components that are not covered by prior high level languages?}
Such features enable rapid development of concurrent and distributed
dataplane applications, such as those that concurrently
monitor and report network health and load, or that engage in distributed
routing, load balancing, caching, failure detection, or security protocols.

% \reminder{Paragraph 1 option 2: migrating the control plane to the data plane.}
% Driven by the emergence of line-rate reconfigurable hardware, control plane tasks are increasingly being migrated to the data plane. This can offer many benefits, such as improved application performance, faster reaction to faults, and enhanced monitoring and security capabilities~\reminder{[cites]}. These \emph{self-controlled} data plane programs are significantly more complex than traditional data plane programs (i.e., focused only on forwarding), with features including recursion, complex control flow, stateful operations, concurrency, and distributed computation~\reminder{cites}.

% \begin{itemize}
% 	\item \textbf{concurrent operations}, which the data plane executes in-between the forwarding of packets;
% 	\item \textbf{stateful operations}, used to implement application-specific data structures;
% 	\item \textbf{recursion}, to update and iterate over data structures;
% 	\item \textbf{complex control flows}, with deeply nested conditional statements; 
% 	\item and \textbf{distributed computation} across multiple data plane nodes.
% \end{itemize}

\OMIT{
It is possible, but challenging, to implement programs with these features in reconfigurable switch hardware. There are two compounding factors: irregular hardware and low-level programming languages. A reconfigurable switch pipeline has many different specialized components, e.g., parsers, match-action pipelines, mirroring engines, queue managers, and configurable MAC blocks. At a finer granularity, some of the components are themselves composed of many different specialized units, e.g., a match-action pipeline contains ALUs, stateful ALUs, hash units, TCAM tables, and SRAM memories.

Today, developers must grapple with this irregularity directly and at a low level of abstraction. Even simple tasks require them to program multiple components, each with their own specific commands and syntax. For example, consider periodically scanning an array, e.g., to determine if a neighboring switch has failed. Implementing this routine in the Barefoot Tofino ASIC requires programming its parser, deparser, reconfigurable memories, stateful ALUs, mirroring engine, and recirculation port. Some parts of the routine can be implemented in P4, while others must be implemented as Tofino-specific microcode or encoded as configurations executed by a control server at runtime.

Further, even when developers can use a well-defined language (e.g., P4), they must be intimately familiar with the underlying hardware. Current languages do not enforce hardware constraints at the source level of abstraction and leave many constraint as implicit. Effectively, they make it easier to implement and optimize routines that the developer knows will map to a specific component of the hardware, \emph{but do not help identify or provide feedback for routines that cannot map.}

As a solution, this paper introduces \lang: a high-level language for general-purpose programs on reconfigurable switch hardware. The main design goal of \lang is to make it easier to express and map complex algorithms to irregular switch hardware while also providing feedback to help developers adjust programs that are ill-suited for line-rate execution. 

At its core, \lang is an event-based language with general abstractions such as higher-order functions, recursion, and primitives for inter-node communication. These abstractions are powerful: they make a wide range of algorithms and data structures easier to express. Atop this, \lang introduces a novel type system, syntactic restrictions, and static analysis passes to provide developers with useful source-level errors, warning, and reports for programs that are either unlikely to compile or whose performance is workload dependent. 
}

The \lang compiler analyzes user programs and translates valid programs
into a lower-level intermediate language for optimization.
%targets the Barefoot Tofino.  It demonstrates the practicality of \lang on today's reconfigurable switches. It translates high-level \lang programs into an intermediate representation based on Guarded Command Language (GCL)~\cite{dijkstra1975guarded}, 
At this level of abstraction, it applies a series of classic compiler 
algorithms to optimize code and maximize parallelism. The compiler then
configures our custom runtime system and generates
a P4 program that includes Tofino-specific pragmas to guide layout of state
across a PISA pipeline.  
%Ultimately, it relieves developers from having to program and optimize the many heterogeneous components of a switch's hardware pipeline.

To evaluate \lang, we develop a diverse set of event-driven data plane programs that integrate latency sensitive control loops directly into the data plane hardware. Applications include a stateful firewall, a telemetry service, a DDoS protection system, and a performance aware router. All programs compile to the Tofino and have an average of 5-10X fewer lines of code than P4 equivalents. Application level benchmarks demonstrate the performance and fault tolerance benefits of using \lang to integrate latency-sensitive control loops into the data plane. Finally, micro-benchmarks between syntactically equivalent \lang and P4 functions showed that the \lang compiler allows more complex tasks to fit in the Tofino's match-action pipeline, compared to its native P4 compiler.\dpw{I wasn't quite sure what that last sentence meant.
How are these microbenchmarks structured?}

In summary, the contributions of this paper are: 
\begin{itemize}
	\item \lang, a high-level language that makes it easier to implement complex concurrent and distributed algorithms on irregular switch hardware; 
	\item a novel type system, syntactic restrictions, and static analysis passes that identify \lang programs ill-suited for the underlying hardware and provide actionable source-level developer feedback;
	\item a \lang compiler targeting the Barefoot Tofino, which shows how general-purpose event-based abstractions can be implemented and optimized on today's reconfigurable switch hardware using classical compiler techniques; and
	\item an evaluation of \lang with a diverse set of event-driven data plane applications implemented for the Tofino. 
\end{itemize}

\dpw{Somewhere early we should mention that we don't always succeed in getting
things to compile -- a programmer can still write too much logic to fit
in a pipeline.}

% first draft (before 12/20/20) of intro.

% As a solution, this paper introduces \lang: a high level language for complex, self-controlled data planes. At its core, \lang is an imperative language with simple programming and cost models that are designed to be familiar to systems programmers. Atop this, we introduce general abstractions such as higher-order functions, event-driven recursion, and primitives for inter-node communication that make powerful, complex applications easy to develop.

% There are two main challenges for \lang. First, giving developers the flexibility to 
% build complex applications for data plane ASICs \emph{without requiring them to have intimate knowledge of architectural details.} \lang achieves this by providing a completeness guarantee: any \lang program that type checks can compile to a data plane ASIC with sufficient pipeline stages. We provide this guarantee by introducing a linear type system for data plane programs, which reasons about both the order in which stateful variables are used and the types of functions that may access them. 

% The second challenge for \lang is compiling high level imperative code to efficient P4 that runs on real hardware. The \lang compiler, which targets the Barefoot Tofino, leverages an intermediate representation for data plane programs based on Guarded Command Language (GCL)~\cite{dijkstra1975guarded}. Using this representation, the compiler applies classical techniques to both optimize and simplify programs, so that the resultant P4 code has a high degree of parallelism (e.g., it requires few pipeline stages) and can compile without manually-added pragmas (e.g., to specify which stage each P4 table should go into).

% An important feature of \lang is completeness: any \lang program that passes type checking can compile to a data plane with sufficient pipeline resources. This is enabled by a combination of a linear type system, which reasons about the order in which stateful variables are accessed, and restrictions on the functions that can be used to operate on those stateful variables. 

% Our compiler, which targets the Barefoot Tofino, shows how to compile high level 
% imperative code to efficient P4 that runs on real hardware. The compiler introduces an intermediate representation for data plane programs based on Guarded Command Language (GCL). Using this representation, the compiler applies classical techniques to both optimize and 
% simplify programs, so that the resultant P4 code requires fewer stages and can compile 
% without manually-added pragmas.

% To evaluate \lang, we used it to implement several self-controlled data plane applications, including a stateful firewall, a telemetry service, a distributed DNS DDoS protection system, and a performance aware routing system. All programs compiled efficiently to the Tofino and, compared to P4 implementations, had an average of 5-10X fewer lines of code. Application level benchmarks demonstrated the performance and fault tolerance benefits of using \lang to implement latency-sensitive control plane tasks in the data plane. Finally, micro-benchmarks between syntactically equivalent \lang and P4 programs showed that the \lang compiler allowed more complex tasks to fit in the Tofino pipeline, compared to the Tofino's native P4 compiler. 

% In summary, the contributions of this paper are: 
% \begin{itemize}
% 	\item a study of self-controlled data plane programs to identify the characteristics that make them challenging to implement with P4;
% 	\item \lang, a high level language for self-controlled data plane programs based on a novel linear type system;
% 	\item the \lang compiler, which adapts classical compiler techniques to improve resource utilization and automate program layout in data plane pipelines; and
% 	\item an evaluation of \lang with several motivating applications targeting the Barefoot Tofino.
% \end{itemize}


==> sections/old/intro2.tex <==
\section{Introduction}
Modern networks are remarkable distributed computing platforms.  They contain 
hundreds or thousands of individual devices (switches), with each device containing
a reservoir of local compute and storage, and capable of processing billions packets per second~\cite{?}.  Moreover, thanks to the development of new open, programmable switches,
creative engineers can now customize and repurpose that infrastructure to improve
the efficiency of traditional networking functions and to take on new tasks.  Indeed, 
both industry and academia 
have generated a raft of new ideas on how to do so, ranging from deployment of new network management services
such as in-network telemetry~\cite{?}, dynamic security monitoring~\cite{?}, failure detection and recovery~\cite{?}, load balancing and traffic engineering~\cite{?} to development of higher-level services such as application-layer caches~\cite{netcache}, coordination services~\cite{networkpaxos,netchain?} and reliable, distributed virtual functions~\cite{swishmem}.  

Unfortunately, despite this potential, the development of 
new applications is slow, error-prone, and exceedingly difficult. Programmers continue
to grapple with two key problems:

\begin{enumerate}
    \item[(i)] Existing programming infrastructure lacks abstractions for communication and
    coordination across program components, either on a single device, or across
    many devices in a network.
    \item[(ii)] Many simple imperative programs cannot be compiled to irregular switch hardware.
\end{enumerate}

\paragraph*{(i) Communication and Coordination}
Most network applications consist of a collection of interdependent processes.
For instance, at a high level of abstraction, a packet forwarding process requires a routing process and a failure detector to compute available paths.  A traffic engineering
application issues queries to measure load, manages internal state when it receives
results back, and processes new flows as appropriate. 
While some such
processes may be implemented in ordinary software in the control plane, others are better implemented on that irregular switch hardware in data plane. Doing so improve latency and
response times.  Indeed, a host of recent projects~\cite{conga,hula,contra} illustrate
the performance benefits of in-network traffic engineering and load balancing.  
Others propose more efficient, distributed implementations of virtual network functions~\cite{?,?,swishmem}.  And still others, like
NetCache~\cite{netcache}, NetChain~\cite{netchain}, and paxos-in-the-network~\cite{?} show that 
benefits also accrue to higher-level applications when the right components are
relocated to the dataplane.

Ironically, P4, a language designed to program communication infrastructure, 
provides little in the way of abstractions to make it easier to communicate 
information between the dataplane processes needed to manage these varied interdependent tasks.  For instance, to ask one's neighbors for their current load involves
choosing packet format, writing parsers and deparses for the format, 
\dpw{something about queues and groups and broadcast here}, and, of course, editing the
input packet processing pipeline of the current switch and its neighbor.  As another
example, ... \dpw{fill in with example on a single switch, highlight the work that needs to be done --- stateful firewall?} ... recirculation, microcode hacking ... 

\paragraph*{(ii) Irregular Switch Hardware}
Barefoot's Tofino switch is a state-of-the-art programmable ASIC.  It contains 
programmable parsers and deparsers as well as multiple packet-processing pipelines.  Each pipeline contains a series of compute stages, and the stages themselves
contain a gateway table (to dispatch to selected components), ordinary ALUs, stateful ALUs, hash units, containers for packet data and meta-data, TCAM tables, and SRAM memories.  Numerous constraints govern how each component can be used and the way packet data and meta-data can flow between them.

% DPW: P4 allows you to program the hardware but is low-level/verbose
P4~\cite{p4} attempts to protect application developers from some of this complexity
by providing a language for programming parts of this hardware and a compiler to 
generate low-level code for specific hardware targets.  The P4 language 
contains some familiar components such as imperative variables, arrays, conditionals and
sequencing.  Hence, it appears one can easily craft simple C-like code to achieve a variety of goals.  Unfortunately, appearances are often deceiving
as simple, valid P4 statements and expressions sometimes fail 
to compile due to the underlying hardware constraints.  For instance a simple conditional like the following one
will not compile with \dpw{Put compiler version here} because the combination of
a subtraction and a comparison will not fit in a Tofino gateway table.
\begin{verbatim}
    if (current - last > THRESHOLD) { ... }
\end{verbatim}
Hence, P4 tries to provide the abstraction of a simple, uniform imperative language, but the
irregular hardware constraints leak through the abstraction barrier to the programmer,
causing unexpected, confusing failures.
Moreover, because P4 is intended to be hardware-independent, the language definition
itself does not explain why such failures occur.  Programmers are usually left
to try to infer what is wrong with their program from the low-level
\emph{outputs} of the compiler, such as the number of hardware stages
generated \dpw{what else do you get other than hardware stages? better example needed here}, rather than being given direction, constraints, or error messages 
in terms of the \emph{source program} they have constructed.

\dpw{I was tempted to add text about Lyra, Chipmunk, etc here but it felt out of place
and/or brought the argument in the wrong direction because we had not yet unveiled our
solution.  I'm wondering about a short section 2 related work on languages like Lyra.}

\noindent
\paragraph*{\lang:  Simple, Event-driven Programming}
In this paper, we introduce \lang, a new, high-level programming
language for Barefoot Tofino, designed to build complex, high-performance dataplane applications. \lang programs are organized as multiple collaborating components
located either on a single device or distributed across many devices in a network.  
To communicate between components, users declare and program with high-level, abstract \emph{events}.  Each such event is named and carries data of the declared type.  Events are also associated with \emph{times} and \emph{locations} to facilitate communication between components both here (on the same switch) and now (immediately), 
as well as across a network, amongst all ones neighbors, and/or perhaps delayed until a little later.  Events also allow communication between \lang components, and regular, perhaps legacy, P4.  These high-level abstractions allow users to construct applications 
with complex control flow and sophisticated, distributed coordination patterns trivially
without having to worry about the low-level details of custom packet formats,
parsers and deparsers, microcode for queuing and recirculation or having to "roll their own" mechanisms for buffering and delayed information processing.\dpw{gotta back that up with examples later in the paper ...}.

\lang's features for coordination between concurrent components are complimented by a careful "correct-by-construction" design of the language for programming the components themselves.  Rather than giving programmers permission to write arbitrary code that then fails to compile, \lang uses several techniques in concert to avoid, or to detect and respond to programmer errors at the source language level of abstraction:

\begin{enumerate}
    \item \textbf{Syntactic constraints}: We define domain-specific,
    source-language constraints to characterize \emph{memops}, the 
    stateful operations that can be executed in a single stage of a pipeline of the Tofino.
    Operations that cannot be executed in a single stage are not classified
    as memops.  Source-level error messages point out exactly where any
    such mistakes occur, making them relatively easy to understand and fix.
    \item \textbf{Types and effects}: We develop a novel 
    \emph{ordered type-and-effect system} that
    limits the way programs interact with persistent memory.  Since persistent
    memory must be allocated to a particular stage of a packet-processing
    pipeline, access to the memory in inconsistent orders by different
    components of a program is impossible to compile without
    recirculation (a costly mechanism that cannot be invoked at line rate).
    Our ordered type system has been designed to support type inference,
    freeing programmers from the need to use complex type annotations,
    while also providing source-level feedback when programming errors occur.
    \item \textbf{Well-designed primitive abstractions}:  We develop
    abstractions for the use of stateful memory such as arrays and
    registers designed to be correct-by-construction.  These abstractions
    may be accessed via interfaces that exploit our domain-specific 
    type system and syntactic constraints.
\end{enumerate}
\noindent
Collectively, these mechanisms help users navigate the difficulty of programming
irregular switch hardware at a high level of abstraction.

\dpw{I wish I could find a way to use this maxim:
    "The mark of a good language is not what it keeps in but rather what it leaves out."}


The \lang compiler analyzes user programs and translates valid programs
into a lower-level intermediate language for optimization.
%targets the Barefoot Tofino.  It demonstrates the practicality of \lang on today's reconfigurable switches. It translates high-level \lang programs into an intermediate representation based on Guarded Command Language (GCL)~\cite{dijkstra1975guarded}, 
At this level of abstraction, it applies a series of classic compiler 
algorithms to optimize code and maximize parallelism. The compiler then
configures our custom runtime system and generates
a P4 program that includes Tofino-specific pragmas to guide layout of state
across a PISA pipeline.  
%Ultimately, it relieves developers from having to program and optimize the many heterogeneous components of a switch's hardware pipeline.

To evaluate \lang, we develop a diverse set of event-driven data plane programs that integrate latency sensitive control loops directly into the data plane hardware. Applications include a stateful firewall, a telemetry service, a DDoS protection system, and a performance aware router. All programs compile to the Tofino and have an average of 5-10X fewer lines of code than P4 equivalents. Application level benchmarks demonstrate the performance and fault tolerance benefits of using \lang to integrate latency-sensitive control loops into the data plane. Finally, micro-benchmarks between syntactically equivalent \lang and P4 functions showed that the \lang compiler allows more complex tasks to fit in the Tofino's match-action pipeline, compared to its native P4 compiler.\dpw{I wasn't quite sure what that last sentence meant.
How are these microbenchmarks structured?}

In summary, the contributions of this paper are: 
\begin{itemize}
	\item \lang, a high-level language that makes it easier to implement complex concurrent and distributed algorithms on irregular switch hardware; 
	\item a novel type system, syntactic restrictions, and static analysis passes that identify \lang programs ill-suited for the underlying hardware and provide actionable source-level developer feedback;
	\item a \lang compiler targeting the Barefoot Tofino, which shows how general-purpose event-based abstractions can be implemented and optimized on today's reconfigurable switch hardware using classical compiler techniques; and
	\item an evaluation of \lang with a diverse set of event-driven data plane applications implemented for the Tofino. 
\end{itemize}

==> sections/old/lang-related.tex <==
\section{Related Dataplane Programming Languages}

Over the past decade, a variety of new dataplane programming languages have been
proposed.  Languages like Frenetic~\cite{frenetic}, NetCore~\cite{netcore}, 
NetKAT~\cite{netKAT}, and McNetKAT~\cite{mcnetkat} allow programmers to specify packet-forwarding paths effectively, but not much more.  In particular,  
they do not have stateful features and hence cannot be used to implement
the same set of dataplane algorithms and applications as \lang.

\dpw{the above is very netkat-centric.  we should mention other things.
Logic programming by Shriram Krishnamurthi.}

More recently, a number of researchers have begun to design higher-level imperative languages for data plane programming including
Chipmunk~\cite{chipmunk}, Domino~\cite{domino}, Lyra~\cite{lyra} and
P4All~\cite{p4all}.  Each of these systems
lifts the level of abstraction at which programmers define their intent
and then uses program synthesis or optimization technology to generate P4- or hardware-level packet-processing pipelines.  In the case of Lyra, these 
pipelines may span multiple devices.  When programmers write programs
that \emph{can} be compiled to the underlying hardware, these technologies work well.  However, when programmers write a program that \emph{cannot be compiled}, something that happens regularly to both
experts and non-experts when navigating the pitfalls of irregular switch hardware, these languages have nothing to say.  Typically, compilation is
attempted with little feedback about what goes wrong when it fails.  In contrast, \lang{} 
defines source-language constraints (using syntax, type systems and
well-defined primitive abstractions) to deliver a "correct-by-construction"
model that avoids the problem of having "valid" source-level programs that
fail to compile.  \lang{} also offers new abstractions for distributed,
event-driven programming.  These abstractions hide low-level Tofino
mechanisms like recirculation and programmable packet queues that 
are not discussed in this other work and would presumably be managed manually.
It seems likely that \lang's correct-by-construction design and abstractions
for distributed, event-driven programming could be added to some of these
other systems.  Conversely, \lang's back-end compiler may benefit from some of 
the program synthesis and optimization technology developed elsewhere.  In
this sense, these research efforts are largely orthogonal and complimentary 
to one another.

Additional related work is discussed in Section~\ref{sec:related}.  
\dpw{Maybe just
plug in all the related work here to save space and avoid breaking it up?}

==> sections/old/motivation.tex <==
\section{Motivation}
\label{sec:motivation}
\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/fault-aware-router.pdf}
\caption {
\exprog architecture. Each data plane node has integrated control loops for fast link failure detection and rerouting. Circles represent tasks, with black arrows for (possibly delayed) control flow. Arrows entering and leaving the box represent unicast or multicast communication with directly connected neighbors. Gray boxes / lines represent state / data access.}
\label{fig:router} 
\end{figure}

\lang is motivated by the challenges of implementing data plane applications with increasingly general characteristics on line-rate switch hardware (e.g., the Barefoot Tofino). The hardware is capable of a surprisingly diverse range of applications, but language- and compiler-related issues make it hard to implement programs with one or more of the following features: complex control flow, iteration or recursion over state, concurrent operations, and distributed computation. 

This section demonstrates the challenges by describing the development of a data plane program with all of the above features. Our example is the \exprog: a destination-based forwarder that integrates control processes for fast in-network link failure detection and rerouting. 

The goal is to detect and route around around failures as quickly as possible. This motivates our design, based on recent work~\cite{hsu2020contra, katta2016hula}, where the control processes are integrated into the data plane. We avoid the inherent latency solutions that place detection and routing in the control plane~\cite{hong2013achieving}, so that our system can react at (or near) the speed of the hardware itself.

%We evaluate a \lang implementation of this program in Section Y.

% \subsection{Fast Rerouting in the Data Plane}
% The main design goal is for network nodes to detect and route around failures as quickly as possible, in a small, bounded amount of time. One possible approach is to use an SDN-based solution, with detection and routing handled outside of the data plane hardware, e.g., at a centralized controller~\cite{hong2013achieving}. However, given the performance objective, this is unappealing because remote control is inherently slow~\cite{hsu2020contra}.

% A more appealing strategy, as recent work has shown~\cite{hsu2020contra, katta2016hula}, is to integrate the detection and (re)routing loops into the data plane program, so that they can execute at (or near) the speed of the hardware itself. 

% An implementation with all tasks running in the dataplane can best meet the performance goal, but such a program is challenging to implement in P4 because it has complex control flow, stateful operations, concurrency, and distributed computation. 

\heading{Program Architecture.} Figure~\ref{fig:router} shows the architecture of the \exprog, which has three main tasks. 

\begin{enumerate}

\item \textbf{Forwarding.} A node forwards packets by looking up a next hop in a route map. Before sending the packet out, the node checks a neighbor status map to see whether the next hop is still reachable (i.e., it has replied to a ping within a threshold period of time). If the next hop is no longer reachable, or if there is no next hop, the node increments a route failure counter for the destination.
\item \textbf{Fault detection.} Interleaved with packet forwarding, a node also regularly pings all of its directly connected neighbors to detect link or node failures. When a neighbor responds to a ping, a node records the time of response in its neighbor status map. 
\item \textbf{Routing.} Concurrent with forwarding and fault detection, each node also periodically scans its routing map to identify destinations that either have no next hop, or a next hop that has become unreachable. When such a destination is found, a node broadcasts a query to all of its neighbors. The neighbors reply with the length of their paths to the destination; the node selects the neighbor with the shortest path length as the destination's next hop.

\end{enumerate}


\subsection{Routing in the Data Plane} 
\label{ssec:p4router}
We start with the \exprog's routing process. Our goal is to implement a straightforward all-pairs shortest path algorithm. Implementing this for the Tofino is remarkably challenging because it involves \emph{inter-device communication} and \emph{persistent computation}, neither of which is well-supported by P4 or other data plane languages. 

% Both of these program features are a challenge to implement in P4. 

\heading{Inter-device communication.} There are two kinds of inter-device messages necessary for route computation. First, a route query that a switch broadcasts to all of its neighbors to requests the current length of the route to a specific destination. Second, a route reply that a switch sends to one of its neighbors in response to a route query. In P4, we represent these messages as \emph{control packets} that are separate from forwarded packets. A control packet stores an instruction (either \emph{route query} or \emph{route reply}) and the appropriate operands as an Ethernet payload. 

While the messages and communication patterns are simple, it is tedious to implement the distribution mechanisms. P4 does not include any high-level primitives for application level inter-device messaging, so we must implement it by programming multiple components of the Tofino at a low level. 

\begin{enumerate}
  \item We define the control packet headers. (X lines of P4)
  \item We implement and integrate the appropriate parse functions. (X lines of P4)
  \item In the match action pipeline, we adjust the control flow to branch based on (1) whether a packet is a control or data packet and (2) which instruction the control packet contains. (X lines of P4)
  \item In either the match action pipeline or deparser, we write a function that generates a control packet.  (X lines of P4)
  \item Finally, we configure the multicast engine to broadcast route query control packets and, if desired, set up queues for guaranteed delivery. (Y lines of Python)
\end{enumerate}

None of these modifications are challenging individually, but there are a lot of moving parts and many fine details to get right. In total, it takes X lines of P4 and Y lines of Python scattered across the program to implement just the distribution mechanisms for route query and reply messages. Wouldn't it be nice if such lines just dissapeared? 

\heading{Persistent in-network computation.}
Route queries, as described above, are triggered by a persistent process that each switch runs to periodically scan for failed routes. The core of this is a simple loop that iterates over the \inl{nextHop} and \inl{lastPing} register arrays to check if each route's next hop is still reachable. Since P4 does not have abstractions for persistent computation or iteration, we must implement this loop with low-level primitives. Packet recirculation is the key enabler: each match action pipeline of the Tofino has a dedicated 100 Gb/s recirculation port. We leverage this to iterate over our data structure by repeatedly recirculating a single control packet containing an index \inl{i}. In each pass through the pipeline, the switch checks \inl{nextHop[i]}, increments \inl{i}, and recirculates the packet. 

Implementing a basic version of the scanning loop amounts to repeating most of the same steps that we followed to implement the inter-node route query and route response messages (i.e., defining the header of the new control message, adding a parser, etc.) One operation, however, is particularly tricky to implement: delay. We would like the ability to ``\emph{pause}'' between executions of the scanning loop, for a reconfigurable length of time, as the specification of the \exprog described. 

The most general solution is to assign instruction packets to a dedicated queue in the recirculation port and pause the queue as needed~\cite{calendarqueues}. Setting up the queuing engine requires configuration from the control plane, while pausing the queue at precise intervals requires either custom driver level code running in the switch's management CPU~\cite{calendarqueues} or sending specially crafted \emph{pause frame packets} to the recirculation port's Ethernet MAC unit. These pause frames can be generated by either a custom program running on the switch's CPU or, for better precision, the Tofino's packet generator, which is also configured by special control plane commands.


\subsection{Forwarding With Register Arrays} 
\label{ssec:p4forwarder}
The \exprog's forwarding process is simple compared to its routing process. However, we still face a myriad of challenges when implementing it for the Tofino. Many of these challenges arise from the fact that we are operating on state that must be read and written from the data plane, i.e., P4 Register Arrays.

For simplicity, we assume that there are a static set of $n$ hosts in the network, with a read-only P4 table that maps each host's IP address to an ID ranging from $1$ through $n$. The remaining task is to implement a P4 control block that maps each host ID to an output port. 

% \inl{control ^Forwarder^(in bit<32> dstId, out bit<32> egrPort)\{}\dots\inl{\}} 

\begin{figure}[t]
\begin{lstlisting}[style=P4Snip]
control ^Forwarder^(in md_t md, in bit<32> dstId, out bit<32> egrPort) {
  Register<bit<32>, bit<32>>(NUM_HOSTS, NO_ROUTE) nextHop;
  Register<bit<32>, bit<32>>(NUM_LINKS, 0) lastPing;
  Register<bit<32>, bit<32>>(NUM_HOSTS, 0) failCt; 
  RegisterAction<bit<32>,bit<32>>(nextHop) getNextHop = {
    void apply(inout bit<32> storedVal, out bit<32> retVal) 
      { retVal=storedVal; }
  };
  RegisterAction<bit<32>,bit<32>>(lastPing) getLastPing = {
    void apply(inout bit<32> storedVal, out bit<32> retVal) 
      { retVal=storedVal; }
  };
  RegisterAction<bit<32>>(failCt) incFailCt = {
    void apply(inout bit<32> storedVal) 
      { storedVal = storedVal+1; }
  };
  apply {
    egrPort = getNextHop.execute(dstId);
    if (egrPort != NO_ROUTE) {
      bit<32> lastPingedTs = getLastPinged.execute(egrPort);
      if (md.ts - lastPingTs > TIMEOUE_THRESH)
        egrPort = NO_ROUTE;
    }
    if (egrPort == NO_ROUTE) {
      incFailCt.execute(dstId);
    }
  }   
} 
\end{lstlisting}
\caption{The forwarding component of \exprog, written in P4\_16-Tofino.}
\label{fig:exprogP4Forward}
\end{figure}

% Simple things are incredibly verbose.
\heading{Simple stateful operations.}
Figure~\ref{fig:exprogP4Forward} shows a basic implementation. P4's verbosity is an immediately obvious issue. Operations over state are particularly complicated to write because in P4, we express a stateful routine (a \inl{RegisterAction}) as an attribute of the state (\inl{Register}) accessed. This abstraction matches how the underlying hardware executes, but is frustratingly low level for programmers.


% Figure~\ref{fig:exprogP4Forward} shows a basic implementation. P4's verbosity and lack of modularity is an immediately obvious issue.  Lines are long because of type annotations. These are necessary because P4 is strongly typed (to reduce programmer errors), but lacks type inference. 
% Operations over state are complicated to write because in P4, we express a stateful routine (\inl{RegisterAction}) as an attribute of the state (\inl{Registers}) accessed. This abstraction matches how the underlying hardware executes, but is frustratingly low level for programmers.

% More discussion about verbosity.
Further, the \inl{RegisterActions} are not re-usable. 
In Figure~\ref{fig:exprogP4Forward}, \inl{getNextHop} and \inl{getLastPing} both do the same thing: simply return a value from memory. However, despite the fact that they are almost identical, we must write two separate copies. \reminder{In total, a P4 implementation of the \exprog contains 81 lines of  register action code to implement four simple stateful operations that are used several times in the program.}
\js{I don't think we need to mention it here, but for comparison, these four operations are 25 lines of code in \lang and can be reused in the code. Also, the entire \exprog is only around 250 LoC in \lang.}

% implicit limitations that make stuff hard to compile. 
\heading{Inferring implicit restrictions.}
Although the P4 code in Figure~\ref{fig:exprogP4Forward} is syntactically valid, it will not compile due to the conditional statement (\inl{if (md.ts - lastPingTs > TIMEOUE_THRESH)}). Compilation will initially fail because the left hand side of the expression is a compound operation that cannot be implemented in the Tofino's gateway tables (i.e., the unit designed to support control flow branching). To fix this, a programmer might try to split the operation into two lines.
\begin{lstlisting}[style=P4Snip]
  bit<32> delta = md.ts - lastPingTs;
  if (delta > TIMEOUT_THRESH) ...
\end{lstlisting}

% Compiler design issues
This will also fail to compile. In the frontend of the P4 compiler, an optimizing pass that is oblivious to the limitations of the Tofino will inline the right hand side of \inl{bit<32> delta = md.ts - lastPingTs;} into subsequent code, silently undoing the attempt to simplify operations. The fix is to encapsulate the statement in an action defined outside of the apply block, which hinders readability.  

% More implicit restrictions
Unfortunately, the compilation will still fail because of a second hardware limitation that is not represented in P4: gateway tables can only support less/greater than comparisons for variables smaller than 12 bits. One possible workaround is using a saturating subtract operation (i.e., one that cannot underflow) to transform the \inl{>} test into a \inl{!=} test. Alternatively, we could restructure the code to perform the test inside of the inside of \inl{RegisterAction getLastPing}. 

% Complex register actions
Either workaround will allow us to compile \inl{^Forwarder^}, but the two alternatives require different numbers of pipeline stages. Embedding the test inside of the register action is the more efficient design. However, complex register actions are also a hazard for programmers. The language that is used to implement register actions is a Tofino-proprietary extension to P4 with an  unrestricted syntax. In this language, it is easy to write actions that are too complex to fit into the underlying stateful ALUs. In some cases, an invalid stateful program \emph{will} compile, but to Tofino assembly code that is either syntactically incorrect or simply wrong. 


\subsection{Summary} 
The \exprog is a sophisticated data plane program that uses integrated control loops for fast fault detection and recovery. The Tofino has all the capabilities necessary to support it, but the implementation is difficult. Several key issues are: verbose and incomplete low-level abstractions, especially for stateful operations; implicit restrictions not represented in the language (or even compiler frontend); and a lack of primitives for inter-device communication and persistent computation. 

Language and compiler issues are the root cause, \emph{rather than the underlying hardware.}

\OMIT{
\subsection{Summary}
The \exprog is a sophisticated data plane program that uses integrated control loops for fast fault detection and recovery. The Tofino has all the capabilities necessary to support it, but the implementation is extremely challenging. Most challenges arise from language and compiler issues, rather than the irregularity of the underlying hardware. 

The P4 language is designed to match the general capabilities of certain components in the Tofino, rather than developer intent. This results in verbose syntax, low level mechanisms, poor modularity, incomplete abstractions, and implicit restrictions that are difficult to infer. Also, since P4 encompasses only a subset of the switch's hardware elements, programmers must implement core operations by configuring parts of the hardware directly, e.g., using pause frames to implement delays. 

The underlying compiler exacerbates these issues because there is a loose coupling between the P4 frontend and the Tofino backend. This causes premature and incorrect optimizations, an implicit binding between P4 constructs and hardware units (e.g., \inl{if/else} statements and gateway tables), limited developer feedback, 
%poor or missing error messages, 
and makes manual optimization and layout necessary in complex programs. 
}


% Challenges: 
% Verbose and low level language
% Lack of modularity
% Implicit restrictions
% Compiler design issues (premature optimizations)
% Incomplete abstractions (for register actions)
% Programming multiple components, specifically for delay. 
% Composing components / threads of a program
% High level constructs unnecessarily bound to specific low-level hardware
% Manual optimization, layout, and variable allocation

% Language: 
% Verbose syntax
% No type inference
% Lack of modularity
% Implicit restrictions
% Incomplete abstractions

% Compiler:
% Premature / incorrect optimizations
% Tight binding between high level constructs and specific low level hardware
% The need for manual optimizations, layout, and variable allocation
% Poor or missing error messages




% In C, we might write this as: 
% \begin{lstlisting}[style=PsuedoSnip]
%   for (int i = 0; i < NUM_HOSTS; i++) {
%     int outPort = nextHop[i];
%     if (time() - lastPing[outPort] > TIMEOUT_THRESH)
%       queryCurrentRoute(SELF, NEIGHBORS, dst);
%   }
% \end{lstlisting}

==> sections/old/motivation_v1.tex <==
% SCRAP (1/4/20)

% \begin{figure}[t]
%   \begin{centering}
%   \begin{multicols}{2}
%   \begin{lstlisting}[style=P4Snip]
%   header ctl_h {
%     bit<8> instr;
%   }

%   header scan_h {
%     bit<32> i;
%     bit<32> delay;
%   }

%   header query_h {
%     bit<32> switch_id;
%     bit<32> dst;
%   }
%   header resp_h {
%     bit<32> switch_id;
%     bit<32> dst;
%     bit<32> pathlen;
%   }
%   \end{lstlisting}
%   \end{multicols}
%   \end{centering}
% \caption{Headers for the routing component of \exprog.}
% \end{figure}[t]

% \begin{figure}[t]
%   \begin{lstlisting}[style=P4Snip]
% apply {
%   if (hdr.ctl.instr == SCAN) {
%     bit<32> outPort = getOutPort.execute(hdr.scan.i);
%     if (outPort =! NO_ROUTE) {
%       bit<32> lastPingedTs = checkTimeout.execute(egrPort);
%       if (checkTimeout == TRUE)
%         queryNeighbors.apply(SELF, hdr.scan.i);
%     }
%     else {
%       queryNeighbors.apply(SELF, hdr.scan.i);
%     }
%     hdr.scan.i = hdr.scan.i + 1;
%     if (hdr.scan.i == NUM_HOSTS) {
%       hdr.scan.i = 0;
%       md.delay = T_WAIT;
%     }
%     md.egrPort = RECIRC_PORT;   
%   }
%   else if (hdr.ctl.instr == QUERY)  {...}
%   else if (hdr.ctl.instr == RESP)   {...}
%   else {...} //handle non instruction packets 
% }  
%   \end{lstlisting}
%   \caption{Excerpts from the \exprog's routing component.}
%   \label{fig:exprogP4Route}
% \end{figure}

% \begin{figure}[t]
%   \begin{lstlisting}[style=P4Snip]
%     apply {      
%       bit<32> outPort = getOutPort.execute(hdr.i);
%       if (outPort =! NO_ROUTE) {
%         bit<32> lastPingedTs = checkTimeout.execute(egrPort);
%         if (checkTimeout == TRUE)
%           queryNeighbors.apply(SELF, hdr.i);
%       }
%       else {
%         queryNeighbors.apply(SELF, hdr.i);
%       }
%       hdr.i = hdr.i + 1;
%       if (hdr.i == NUM_HOSTS) {
%         hdr.i = 0;
%         hdr.delay = T_WAIT;
%       }
%       md.egrPort = RECIRC_PORT;
%     }  
%   \end{lstlisting}
%   \caption{The apply block of a recirculation-based route failure detection loop in P4.}
%   \label{fig:exprogP4Route}
% \end{figure}


\OMIT{
\subsubsection{Routing}
% recap
The routing component has three core tasks: scanning the register arrays for failed routes; querying neighbor switches for route updates; and aggregating query responses from neighbors to find new routes. 

% design overview
We implement these tasks in P4 using using \emph{instruction packets} that are separate from forwarded packets. An instruction packet stores an instruction and operands in a custom header (e.g., a shim header between Ethernet and IP). The Tofino's match action pipeline processes the instruction packets, using an apply block like the one shown in Figure~\ref{fig:exprogP4Route}.

% monolithic, unstructured code
The first issue we observe is the code's lack of structure. Logic for handling all three tasks is interleaved. This is unavoidable. In P4, register arrays are scoped to a single control object and cannot be passed as arguments to other control objects. Thus, since all three tasks use a common set of register arrays, they must all be implemented in a single monolithic apply block.

% forcing developers to use low level primitives
% also describing how we do iteration
The core of the routing component (the \inl{SCAN} branch in Fig~\ref{fig:exprogP4Route}) is a simple loop that periodically scans every routing entry to check if its next hop is still reachable, by iterating over the the \inl{nextHop} and \inl{lastPing} register arrays. Since P4 does not have an abstraction for iteration over state, we must implement it using a low level primitive: packet recirculation. Each match action pipeline of the Tofino has a dedicated 100 Gb/s recirculation port. We leverage this to iterate over our data structure by repeatedly recirculating a single instruction packet containing an index \inl{i}. In each pass through the pipeline, the switch checks \inl{nextHop[i]}, increments \inl{i}, and recirculates the packet. 

% \begin{figure}[H]
% \includegraphics[width=\linewidth]{figures/tofino-pipe.pdf}
% \caption {
% Components in the Tofino that must be programmed to implement the route failure detector in~\ref{fig:exprogP4Route}.}
% \label{fig:tofino-pipe} 
% \end{figure}

% Programming multiple components, specifically for delay. 
The routing component is complicated to implement in large part because it relies on careful programming and configuration of components outside of the match action pipeline. Several of these components are not represented in P4. For example, consider the delay operation, i.e., delaying recirculation of the \inl{SCAN} instruction packet by \inl{T_WAIT} each time the scanning loop restarts. The most general solution is to assign instruction packets to a dedicated queue in the recirculation port and pause the queue as needed~\cite{calendarqueues}. Setting up the queue require configuring the switch's queuing engine from the control plane, while pausing the queue at precise intervals requires sending specially crafted \emph{pause frame packets} to the recirculation port's Ethernet MAC unit. These pause frames can be generated by either a custom program running on the switch's CPU or, for better precision, the Tofino's packet generator, which is also configured by special control plane commands.

% Programming the more mundane components. 
Additionally, to implement the route scanning loop, we must write parser and deparser functions for the instruction packets and configure the multicast engine to enable \inl{queryNeighbors}. If we want to ensure that instruction packets are not dropped due to data plane congestion, we must also configure queue priorities for both the recirculation port and also the ports connected to neighboring nodes. 

\subsubsection{Composing Forwarding and Routing}
\js{This section can probably use more concrete examples.}


% many different functions to integrate
Composing the forwarding and routing components is difficult. There are multiple parts of the code that must be integrated: the parsers, deparsers, and the match action pipeline that implements control objects (e.g., Figure~\ref{fig:exprogP4Forward}). 

Composing the match action pipeline is challenging because of issues related to \emph{branching statements}, \emph{register arrays}, and \emph{register actions}, which arise as the complexity of a match action pipeline increases. 

% limited modularity of control blocks (promoted to routing subsubsec)
% Control objects are hard to compose because of P4's scoping rules. Register arrays are scoped to individual control objects and cannot be passed as parameters. For programs like the \exprog, which has multiple components that share the same state, we must combine all components into a single control object with a complex monolithic \inl{apply} block.

% Implementing complex programs in P4 is challenging because of issues related to \emph{branching statements}, \emph{register arrays}, and \emph{register actions}.

% Interleaving the execution of these threads is trivial because the Tofino's pipelined architecture guarantees that packet operations are atomic~\cite{domino}.

% gateway table and branch complexity.
\heading{Branching statements.}
As we merge more components of an application into a single control object, the apply block grows more complex in terms of how many conditional branches there are and how deeply they are nested.
An issue arises with such complex control flows. The gateway tables that implement \inl{if/else} statements can only encode a small, limited number of conditionals. So, when a control flow becomes sufficiently complex, the program will fail to compile. 

% manual optimizations
An alternative strategy is to branch with \texttt{switch} statements. A switch statement uses a full match action table to select the next statement based on which action the table applies. Full match action tables do not have the limitations of gateway tables and can encode extremely complex conditionals~\cite{maple}. 
However, applying a match action table is more expensive. To fit functions with long critical paths (e.g., more than $\approx$10 sequential operations) in the Tofino's match action pipeline, programmers must structure their program so that the operations immediately following a \inl{switch} statement are done inside of the switch table's actions. 

% memory access order
\heading{Register arrays.}
As a consequence of the Tofino's stage-local memories, every execution path of a P4 program must access registers in the same order. This is easy to enforce in small programs, but quickly becomes tedious as complexity increases. Further, inconsistent ordering can cause failures that arise in late stages of compilation and produce errors that are difficult to decipher. For example, in complex programs with inconsistent ordering we have experienced faults that arose after 10+ minutes of compilation in the match-action table layout stage, which is deep in the Tofino compiler's backend.  

% annotations or manual optimizations
Additionally, when programs access the same state from different execution paths, it becomes more difficult for the compiler to find a feasible layout of instructions. For complex programs, compilation only succeeds with either: 1) manually added pragmas, denoting the physical stage of each table; or 2) manual optimization of program structure to eliminate branches. 

% multiplexing salus
\heading{Register actions.} 
A programmer must manually multiplex memory ports in the underlying hardware to successfully compile programes with multiple independent control paths that perform different operations on the same register arrays. In the Tofino, all the register actions for a single register compile to one stateful alu (sALU). A sALU has has two input ports. Thus, if the actions of a register array reference more than two metadata fields in total, a programmer must manually resolve the issue by mapping all the metadata fields to at most two temporary variables. 

}



\section{Motivation}
\label{sec:motivation}
\begin{figure}[H]
\includegraphics[width=\linewidth]{figures/fault-aware-router.pdf}
\caption {
Architecture of a data plane node with integrated control loops for fast link failure detection and rerouting. Circles represent tasks, with black arrows for (possibly delayed) control flow. Arrows entering and leaving the box represent unicast or multicast communication with directly connected neighbors. Gray boxes / lines represent state / data access.}
\label{fig:router} 
\end{figure}

\lang is motivated by the challenges of implementing data plane applications with increasingly general characteristics on line-rate switch hardware (e.g., the Barefoot Tofino). In our experience, the hardware is capable of supporting a surprisingly diverse range of applications, but language- and compiler-related issues make it hard to implement programs with one or more of the following features: complex control flow, iteration or recursion over state, concurrent operations, and distributed computation. 

To explain more concretely, this section describes the challenges that arise when developing a data plane program that integrates control loops for fast in-network link failure detection and rerouting. We evaluate a \lang implementation of this program in Section Y.

% , along with the other motivating applications in Table X.

% \begin{table}[!t]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}
% \begin{tabularx}{\linewidth}{ l l l l l } 
% \toprule
%  \textbf{Application} & \textbf{Ctl. Flow} & \textbf{Sfl. Ops} & \textbf{Concurrency} & \textbf{Distr. Comp.} \\
%  \midrule
%  \textbf{TurboFlow} & check & check & - & - \\
%  \textbf{DNS Defense} & check & check & check & - \\
%  \textbf{Stateful FW} & check & check & check & - \\
%  \textbf{Fault Aware Rtr} & check & check & check & check \\
% \bottomrule
% \end{tabularx}
% \caption{Features of advanced dataplane applications.}
% \label{tab:usecases}
% \end{table}



% Table X: 
% application    		| control | state | concurrency | distributed
% TurboFlow   			| check   | check | -           | - 
% DNS Defense 			| check   | check | check       | - 
% Stateful FW 			| check   | check | check       | -
% Fault aware router 	| check   | check | check       | check


\subsection{Fast Rerouting in the Data Plane}
The main design goal is for network nodes to detect and route around failures as quickly as possible, in a small, bounded amount of time. One possible approach is to use an SDN-based solution, with detection and routing handled outside of the data plane hardware, e.g., at a centralized controller~\cite{hong2013achieving}. However, given the performance objective, this is unappealing because remote control is inherently slow~\cite{hsu2020contra}.

A more appealing strategy, as recent work has shown~\cite{hsu2020contra, katta2016hula}, is to integrate the detection and (re)routing loops into the data plane program, so that they can execute at (or near) the speed of the hardware itself. 


% An implementation with all tasks running in the dataplane can best meet the performance goal, but such a program is challenging to implement in P4 because it has complex control flow, stateful operations, concurrency, and distributed computation. 

\subsubsection{Program Architecture}

Figure~\ref{fig:router} shows the architecture of our desired data plane program, which has three main tasks. 

\begin{enumerate}

\item \textbf{Forwarding.} A node forwards packets by looking up a next hop in a route map. Before sending the packet out, the node checks a neighbor status map to see whether the next hop is still reachable (i.e., it has replied to a ping within a threshold period of time). If the next hop is no longer reachable, or if there is no next hop, the node increments a route failure counter for the destination.
\item \textbf{Fault detection.} Interleaved with packet forwarding, a node also regularly pings all of its directly connected neighbors to detect link or node failures. When a neighbor responds to a ping, a node records the time of response in its neighbor status map. 
\item \textbf{Routing.} Concurrent with forwarding and fault detection, each node also periodically scans its routing map to identify destinations that either have no next hop, or a next hop that has become unreachable. When such a destination is found, a node broadcasts a query to all of its neighbors. The neighbors reply with the length of their paths to the destination; the node selects the neighbor with the shortest path length as the destination's next hop.

\end{enumerate}

\subsubsection{Program Features}
\label{ssec:progfeatures}
It is easy to imagine developing the example application, given a few basic abstractions that are either built-into or easy to implement in virtually all general-purpose programming languages. 

\dpw{At first glance (before reading future sections), it actually seems like
P4 can handle several of these things just fine -- it has nested conditionals
(I take your point about the gateways, but almost no reader will recognize
that yet and will instead say "but P4 has gateways"; it has stateful functions;
it can process multiple packets in a pipeline and so it has concurrency.
So it feels, at this point, like most of this section doesn't point to new things in our
design (even though it eventually will).}


\begin{itemize}
	\item {\textbf{Iteration.} The routing and fault detection control loops repeatedly scan the entries in the route and link status maps, which is easy to express as iteration.}
	\item {\textbf{Nested conditional branching.} Each task of the router has multiple execution paths that are selected conditionally, dependent on variables that are evaluated at different points in the program. This control flow is easy to express with nested \texttt{if/else} statements.}
	\item {\textbf{Stateful functions.} Interleaved with branching operations are reads and writes to the route and neighbor status maps. Multiple components of the router execute the same sequences of operations, which are naturally abstracted as stateful functions. For example, routing and forwarding both read the next hop associated with a destination from the route map.}  
	\item {\textbf{Concurrency.} All three tasks (forwarding, routing, and fault detection) must take place concurrently, operating on the same shared maps. However, not all of the tasks occur at the same rate. The route and link status check loops, for example, may wish to pause between scanning their respective maps, depending on the operator's requirements. Abstractions for cooperative multi-threading would make this easy to express.}
	\item {\textbf{Distributed computation.} Route computation in the example program is a distributed all-pairs shortest paths algorithm. Fault detection is also an inherently distributed task. Simple primitives for one-to-one and one-to-many messaging would provide the last remaining abstraction necessary for implementing the motivating example.}
\end{itemize}

% Delayed execution? 


\subsection{A Tofino Implementation}

\begin{figure}[H]
\includegraphics[width=\linewidth]{figures/tofino-pipe.pdf}
\caption {
Pipeline of the Barefoot Tofino. Blocks show distinct hardware units and are annotated with symbols showing how each unit is programmed. }
\label{fig:tofino-pipe} 
\end{figure}

Can we actually implement the fault aware router on line-rate reconfigurable switch hardware (i.e., the Tofino)? 
As Section Y will show, it is easy with \lang because it has general-purpose abstractions for all of the features described above. 

Using only the languages currently available for the Tofino, however, makes implementing the fault aware router a daunting challenge. P4, the standard language for programming the Tofino, does not have abstractions for most of the above features. Worse, some of the features cannot even be \emph{implemented} in P4 (or any language that compiles to P4) because they require programming components of the switch hardware that are \emph{outside the scope of P4}. 

Figure~\ref{fig:tofino-pipe} shows all the components of the Tofino's pipeline that must be programmed to implement the five core features from Section~\ref{ssec:progfeatures}. Below, we summarize how each feature can be implemented in the Tofino and describe some of the challenges that arise. 

\subsubsection{Iteration}
Because the Tofino can only access each memory location once per packet, iteration over persistent state (e.g., the link status map) must be implemented via packet recirculation. A developer writes a `\emph{stateful action}' (in a Tofino-proprietary P4 extension) that processes one entry of the array per packet, and P4 blocks to parse, deparse, and select an output port for each recirculated packet. These blocks must then be manually composed with any other P4 code. 


\subsubsection{Nested Conditional Branching}
\label{ssec:conds}
The easiest way to conditionally branch in a P4 program is via \texttt{if / else} statements in a P4 control block. However, in the Tofino, this statement has very specific semantics: it programs a small \emph{gateway table} at the beginning of each match+action stage, to select which match action tables get applied. The gateway tables are small, which means that programs whose control flows are too complex, either in terms of number of branches or size of the variables tested in branch expressions, will fail to compile. 

An alternative strategy is to conditionally branch with a \texttt{switch} statement that applies a full match action table and chooses a control flow based on which action was selected. Full match action tables are not subject to the constraints of gateway tables and can encode extremely complex conditionals~\cite{maple}. However, switch statements are less efficient because applying the switch table consumes a match-action stage. Thus, to fit functions with long critical paths (e.g., more than $\approx$10 sequential operations) in the match action pipeline, developers must structure their program so that the operations immediately following the branch are done inside of the switch table's actions.


\subsubsection{Stateful Functions}
\label{ssec:sfuns}
In the Tofino, operations on persistent state are implemented via \emph{stateful actions} written in a Tofino-proprietary P4 extension. A stateful action gets attached to a stateful ALU, which can hold a limited number of stateful actions. Each stateful ALU is bound at compile time to a single block of memory (a \emph{register array} in P4) in a single match action unit. 

Many challenges arise from stateful operations, which we classify as related to either the abstraction of stateful actions or how they are integrated into complex programs. 

\paragraph{\textbf{Stateful actions.}}
First, stateful actions are not re-usable. A stateful action is bound to a single memory and SALU. If the developer wants to perform the same stateful operation, but on a different memory or in a different control flow of the program, they must re-write the stateful action. This hinders readability and code re-use. 

Second, salus only have a limited number of input and output ports. If the stateful actions that map to a SALU use too many input or output variables, a developer may need to manually add and set temporary intermediate variables to multiplex the SALU's i/o ports. 

Finally, and perhaps most importantly, the language that is used to program stateful actions has an unrestricted syntax that makes it easy to write stateful actions that are too complex to fit into a stateful ALU. In some cases, an invalid stateful program \emph{will} compile, but to Tofino assembly code that is invalid. 

\paragraph{\textbf{Integrating stateful actions.}}
As a consequence of the Tofino's stage-local memories, P4 programs that target the Tofino must ensure that they always access register arrays in the same order. This is easy in small programs, but quickly becomes tedious as programs grow more complex. Further, inconsistent ordering can cause failures that arise in late stages of compilation and produce errors that are difficult to decipher. For example, in complex programs with inconsistent ordering we have experienced faults that arose after 10+ minutes of compilation in the match-action table layout stage, which is deep in the Tofino compiler's backend.  

Additionally, when programs access the same state from tables in different branches, it becomes more difficult for the compiler to find a correct layout of match-action tables. For complex programs, compilation only succeeds with either: 1) manually added pragmas, denoting the physical stage that each match action table should be placed into; or 2) manual optimization of program structure to remove branches and combine mutually exclusive operations into the same tables. 

\subsubsection{Concurrency and Distributed Computation}
Programs with concurrency and distributed computations present two main challenges: programming parts of the hardware outside the scope of P4 and composing code for mutually exclusive threads. 

For programs with concurrent threads, an important capability is being able to ``pause'' one thread (e.g., the route check loop in the fault-tolerant router). The most efficient way to do this is by assigning the process a dedicated queue of the recirculation port and pausing it as needed. Setting up the queue require configuring the switch's queuing engine from the control plane, while pausing the queue (at fine timescales) requires sending specially crafted \emph{pause frame packets} to the recirculation port's Ethernet MAC unit. These pause frames can be generated by another component of the Tofino, its packet generator, which is also configured by special control plane commands. 

Additionally, programs with distributed computation may need to broadcast the same message to multiple nodes, e.g., the route check loop queries all of its neighbors for a new route when it identifies a failure. This requires programming the Tofino's multicast and mirroring engines from the control plane. 

The second challenge for concurrent and distributed programs is composing the parsers, deparsers, and match action control blocks from different threads. Assuming that threads are executed by mutually exclusive sets of packets, as in our motivating example router, the task seems conceptually straightforward because the Tofino's pipelined architecture guarantees that memory operations are atomic~\cite{domino}. However, in practice, composition remains challenging because it make control flow more complex and increases the number of memory operations, which give rise to the issues described in Sections~\ref{ssec:conds} and~\ref{ssec:sfuns}.




% pausing - 
% priorities for traffic
% interleaving the logic for concurrent threads, complicates the issues related to branching and stateful operations that were described above. 
% 

% multicast engine configuration
% 


% None of the above abstractions are available in P4, worse they are either difficult or impossible to implement in P4. 

% Go through challenges of implementing each individual abstraction in P4. 

% not all of the above tasks can be implemented in P4. 
% some require configuration of other blocks in the pipeline. 


% "P4 capabilities are more a result of instruction design rather than language design."


% As Section Y will show, it is easy with \lang. However, in P4, we found it to be nearly impossible. The hardware is complex and irregular, with many platform specific limitations that are not explicitly enforced in P4. In practice, developers must learn intricate details about the underlying 
% hardware and \emph{try} to write P4 code to match. The nuances of a specific platform are often only discovered as a program grows more complex. Resolving them requires a combination of trial and error, close reading of low-level architecture documentation, and deciphering the cryptic output of a closed-source compiler. Below, we describe some of the challenges that arose in our attempt to implement the fault-tolerant router in P4.

% \begin{enumerate}
% \item invalid state ordering
% \item incorrect expression folding
% \item gateway table limitations / if-else statements
% \item switch statement overhead
% \item layout failure
% \item manual instruction level optimizations
% \item stateful routine compilation failure
% \item salu register allocation failure
% \item limited code reuse
% \item manual recirculation management (queueing, timing, mirroring, multicasting, parsing, deparsing)
% \end{enumerate}

% Notes on possible applications [11/20]
% \reminder{This section has three purposes: 
% \begin{enumerate}
% 	\item motivate moving tasks from the control plane to the data plane; 
% 	\item highlight the ways that self-controlled data plane programs are complex; 
% 	\item explain why these features make the programs hard to implement in P4.
% \end{enumerate}
% }

% \subsection{Flow-oriented Services} 
% Applications that operate on dynamically-arriving flows. These services are the foundation of today's networks, but are still extremely challenging to implement in a line-rate ASIC. Examples: Stateful firewalls, MAC learners, NATs, Header compression. 

% \subsection{Telemetry} 

% Modern telemetry systems use the data plane to aggregate and stream network measurements to analytics systems. The data plane component significantly reduces the workload of the backend software, allowing it to scale to larger networks. Some example applications include the data plane components of TurboFlow, StarFlow, Speedlight, TPProf, and many system's from Jen's group. 

% \subsection{Learning Systems} 

% Applications that identify flows which must be treated differently from normal traffic and apply advanced actions to them. 
% An example that we are working on in another project: protecting hosts against DNS-based DDoS attacks with a count-min sketch plus a bloom filter acting as an approximate stateful firewall. The sketch recognizes hosts under attack; traffic to and from those hosts is routed to the stateful firewall, which stops the attack traffic with high probability. 


% \subsection{Distributed Systems} 
% In many systems, part of the application is distributed across multiple data plane nodes. 

% \paragraph{Performance aware routing} Data plane nodes react to changes that occur elsewhere in the network. E.g. contra.

% \paragraph{Distributed services} Flow-oriented services that operate over multiple nodes as though they are one big switch. E.g. distributed stateful firewall.


% \subsection{In-network Compute} 
% Hadoop, map-reduce, or memcache in DPT. In-network compute is about migrating services that usually run at the end host into the network.


==> sections/old/overview.tex <==
\section{Introducing \lang}


\lang is a programming language for the Intel Tofino that directly addresses the language and compiler related challenges describe in the previous section. 

Three main components: 

Abstractions for control

Syntactic checks for state ordering and operation constraints

Optimizing compiler

==> sections/old/overview_old.tex <==
\section{The \lang Language}

\reminder{This is homeless content!}



\subsection{Persistent State}
Persistent state is at the core of the \exprog. The forwarding, routing, and fault detection processes all read and write data that persists across packets. 

\lang programs access persistent state through data structure modules. Each module provides a different high-level abstraction over the stateful primitives of the underlying hardware, e.g., arrays, counters, and hash-indexed arrays. This section introduces the core concepts by focusing on how arrays are used in the \exprog.

\subsubsection{Arrays}
The routing component of \exprog accesses arrays that map each host ID to a path length and next hop.
\begin{lstlisting}[style=DptBlock]
global pathlens = new Array<<32>>(NUM_DSTS);
global nexthops = new Array<<32>>(NUM_DSTS);
\end{lstlisting}

These declarations create two arrays (\inl{pathlens} and \inl{nexthops} that each have \inl{NUM_DSTS} 32-bit elements. The arrays are \emph{global}: they persist across packets and can be read or written from any handler or function in the program. 

% The compiler translates this directly into a register array declaration in P4. In a multi-node network, each match action pipeline will have its own instance of \inl{pathlens}.
% The above sentence kind of makes "global" seem like a misnomer.

% \heading{Basic interfaces.}
% We operate on a stateful data structure through methods defined in its module. The most basic methods in the \inl{Array} module are \inl{set} and \inl{get}. For example, the \inl{route_query} handler uses \inl{Array.get} to retrieve the length of the current path to a destination.

% \begin{lstlisting}[style=DptBlock]
% fun int cur_plen(int dst) {return Array.get(pathlens, dst);}
% \end{lstlisting}

\heading{Functional interfaces.}
In \lang, data structure modules provide a powerful functional interface to persistent state. Module methods read values from memory, perform a small amount of computation, and write the results back. For example, the \inl{route_reply} handler needs to compare the length of the path stored in the \inl{pathlens} with the length of the path in the event and save the shorter of the two to memory. We can implement this with one of \inl{Array}'s functional interfaces: \inl{Array.set}.

\begin{lstlisting}[style=DptBlock]
handle route_reply(int switch, int dst, int plen){
	Array.set(pathlens, dst, min_plen, plen);
	...
\end{lstlisting}

The last two arguments to \inl{Array.set} are important: \inl{min_plen} is a function that compares two path lengths and returns the shorter of the two. \inl{plen} is a parameter to pass to \inl{min_plen}. \inl{Array.setm} will read \inl{pathlens[dst]}, call \inl{min_plen(pathlens[dst], plen)}, and write its return value back to \inl{pathlens[dst]}, i.e., it will execute \inl{pathlens[dst] = min_plen(pathlens[dst], plen)}.

% // Here is a complex register action that fails and gives a weird error.
% // It is trying to express: only use the new length if its less than half as long as the current length.
% // This salu fails with: 
% // error: RegisterAction c_c too complex
% // newv = new_len + 1;
% control ComplexSalu(inout header_t hdr) {
%     bit<32> rand_num = hdr.ip.src_addr;
%     bit<32> new_len = hdr.ip.dst_addr;
%     Register<bit<32>,_>(128) c1;
%     RegisterAction<bit<32>,_,bit<32>>(c1) c_1={
%         void apply(inout bit<32> value, out bit<32> rv) {
%             bit<32> newv = value;
%             if (value > new_len + new_len) {
%                 newv = new_len + 1;
%             }
%             value = newv;
%         }
%     };
%     apply {
%         c_1.execute(0);        
%     }
% }



\subsubsection{Restricted Memory Operations} 
In P4 (or other languages) it is easy to write stateful functions that cannot compile to hardware because they do too much computation. Debugging these functions is hard because they are often syntactically valid and only raise cryptic errors from the compiler's backend. 

For example, suppose that in the \exprog, we want a \inl{route_reply} handler that only accepts a new route if its path is less than half as long as the current route's. We might attempt to implement this as follows. 
\begin{lstlisting}[style=DptBlock]
fun min_plen_x2(int stored_plen, int new_plen) {
	int updated_plen = stored_plen;
	if (stored_plen > new_plen + new_plen)  {
		updated_plen = new_plen + 1;
	}
	return updated_plen;
}
handle route_reply(int switch, int dst, int plen) {
	Array.set(pathlens, dst, min_plen, plen);
	...
\end{lstlisting}

\inl{min_plen_x2} is too complex of a stateful function for the Tofino. In P4, we could write this as a \inl{RegisterAction}, but upon compilation we would get a cryptic error from the backend: \texttt{error: RegisterAction too complex}. This tells us little about what is wrong with our function, or how to fix it. 

To make debugging easier, \lang restricts the syntax of functions that can be passed to data structure methods. These restricted functions are called \emph{memory operations} (\inl{memops}). Any syntactically correct \inl{memop} can be translated to a P4 \inl{RegisterAction} \emph{that is guaranteed to compile to the Tofino}.

Once we declare \inl{min_plen_x2} as a \inl{memop}, the \lang compiler's frontend will identify two issues: \inl{min_plen_x2} declares local variables and contains an expression that uses an input parameters multiple times.

This guides us to a working implementation of the desired \inl{route_reply} handler, with \inl{plen + plen} outside of the \inl{memop}.

\begin{lstlisting}[style=DptBlock]
memop min_plen(int stored_plen, int new_plen) {
	if (stored_plen > new_plen)  {
		updated_plen = new_plen + 1;
	}
	return updated_plen;
}
handle route_reply(int switch, int dst, int plen) {
	int plen_x2 = plen + plen;
	Array.set(pathlens, dst, min_plen, plen_x2);
	...
\end{lstlisting}


\inl{Array.set} and \inl{Array.get} are syntactic sugar that wraps the more general \inl{Array.update}, which performs a concurrent read and write. In the full \inl{route_reply} handler, we use the update method to access \inl{pathlen} because we need to determine which of the two paths were selected. 

\begin{lstlisting}[style=DptBlock]
memop min_plen(int stored_plen, int new_plen) {
	if (stored_plen > new_plen + 1)
		return new_plen + 1;
	else
		return stored_plen;
}
memop plen_change(int stored_plen, int new_plen) {
	if (stored_plen > new_plen + 1)
		return true;
	else
		return false;		
}
handle route_reply(int switch, int dst, int plen) {
	bool route_changed = Array.update(pathlens, dst, 
	plen_change, plen, min_plen, plen);
	if (route_changes == true) {
		...
\end{lstlisting}

Here, the call to \inl{Array.update} first executes \inl{plen_change} to calculate a return value, then executes \inl{min_plen} to conditionally update the stored path length. 


\subsubsection{Ordering Constraints}
The \exprog, stores path lengths and next hops in two different arrays. 
\begin{lstlisting}[style=DptBlock]
global pathlens = new Array<<32>>(NUM_DSTS);
global nexthops = new Array<<32>>(NUM_DSTS);
\end{lstlisting}

When a program uses multiple persistent objects, all of its execution paths must access the objects in the same order. This a fundamental constraint of the Tofino because it stores persistent state in stage-local memories that a packet cannot revisit during its processing.

For example, the following \inl{route_query} and \inl{route_reply} handlers violate these constraints. 

\begin{lstlisting}[style=DptBlock]
handle route_query_bad(int sw, int dst) {
	int next_h = Array.get(nexthop, dst);
	if (next_h != NO_ROUTE) {
		int pathlen = Array.get(pathlen, dst);
		event reply = route_reply(SELF, dst, pathlen);
		generate Event.locate(reply, sw);
	}
}
handle route_reply(int sw, int dst, int plen) {
	bool changed = Array.update(pathlens, dst,...);
	if (changed == true)
		Array.set(nexthop, dst, sw);
}
\end{lstlisting}

The \inl{route_query_bad} handler checks \inl{nexthops} before \inl{pathlens}, to ensure that it only generates a response when it knows a route. The \inl{route_reply} handler uses the arrays in the opposite order. It accesses \inl{pathlens} first, to figure out whether or not to update the nexthop for \inl{dst}. As written, these two handlers are impossible to compile without recirculation. 

In P4, it is up to the programmer to keep track of whether state is accessed in a consistent order. Compilation will fail when the constraint is violated, but the resulting error may be deep in the compiler's backend and seemingly unrelated. 
% For example, inconsistent state ordering can sometimes cause the compiler's layout stage to enter a loop where it repeatedly tries to resolve the inconsistency by using more pipeline stages. Ultimately it fails, reporting that the program uses too many pipeline stages.

In \lang, the type system explicitly checks for ordering consistency. It enforces the property that \emph{persistent objects are always used in the order that they are declared.} Assuming \inl{pathlens} was declared before \inl{nexthops}, the resulting error would be \texttt{error: pathlens was declared before nexthop, but handler route_query_bad uses them in the opposite order}.

We can resolve the issue by changing \inl{route_query} so that it accesses the arrays in the same order as \inl{route_reply}. 

\begin{lstlisting}[style=DptBlock]
global pathlens = new Array<<32>>(NUM_DSTS);
global nexthops = new Array<<32>>(NUM_DSTS);
handle route_query(int sw, int dst) {
	int pathlen = Array.get(pathlens, dst);
	int next_h = Array.get(nexthops, dst);
	if (next_h != NO_ROUTE) {
		event reply = route_reply(SELF, dst, pathlen);
		generate Event.locate(reply, sw);
	}
}
handle route_reply(int sw, int dst, int plen) {
	bool changed = Array.update(pathlens, dst,...);
	if (changed == true)
		Array.set(nexthop, dst, sw);
}
\end{lstlisting}

Now, both handlers use \inl{pathlens} and \inl{nexthops} in the order that they are declared, which satisfies the type checker and makes compilation possible. 


\lang also enforces ordering when functions are involved, which is more complicated. For example, we may want a more sophisticated \inl{route_query} that only replies if it has a route shorter than an event-provided threshold. In \lang, we can encapsulate this test in a function.

\begin{lstlisting}[style=DptBlock]
global pathlens = new Array<<32>>(NUM_DSTS);
global nexthops = new Array<<32>>(NUM_DSTS);
fun int get_nexthop(Array nhops, Array plens, int dst, int minlen) {	
	int plen = Array.get(plens, dst);
	if (plen > minlen)
		return NO_ROUTE;
	else
		return Array.get(arr, idx);		
}
handle acceptable_route_query(int sw, int dst, int minlen) {
	int next_h = get_nexthop(nexthops, pathlens, dst);
	if (next_h != NO_ROUTE) {
	...
\end{lstlisting}

Here, \inl{get_nexthop} returns \inl{NO_ROUTE} for \inl{dst} unless the route is shorter than \inl{pathlen}. Verifying that the ordering is consistent is harder for the \lang type checker in this example. The type checker cannot simply look at \inl{get_nexthop} and determine whether ordering is consistent because it doesn't know when the function will be called, or which arrays will be passed to it. \lang resolves this issue by tracking feasible variable orderings while performing regular type inference. 


==> sections/old/overview_scrap.tex <==



% These abstractions let developers program the diverse and heterogeneous components of switch hardware at a high level and in a single, well-defined language. 
The abstractions themselves are carefully designed to be not only simple and familiar, but also to match the capabilities and execution model of the underlying hardware. 

simple, to meet the needs of the developer, but also carefully designed to match the capabilities and execution model of the underlying hardware. 

match not only the needs of the developers, but also the capabilities and execution model of the underlying hardware. 

that are implemented by programming the diverse heterogeneous components of switch hardware.

First, \lang makes it easier to express complex algorithms and data structures that run on switch hardware, by introducing a unified set of general-purpose abstractions. These abstractions 

 by introducing high-level general-purpose abstractions. These abstractions provide a unified 

by introducing a unified set of high-level general-purpose abstractions. 

Our strategy to accomplish this has two complementary parts. 

First, \lang makes it easier to express complex algorithms and data structures by introducing a unified set of high-level general-purpose abstractions that leverage the diverse heterogeneous components of a switch's reconfigurable ASIC. These abstractions are carefully designed to match not only the needs of the developers, but also the capabilities and execution model of the underlying hardware. 

Second, \lang helps developers 

introduces a novel type system, static analysis passes, and emulation-based programming environment 



match the needs of the developers and also the capabilities of the underlying hardware

unified abstraction over the diverse heterogeneous hardware in the switch, so that it can be programmed at a high level and with general-purpose abstractions. 

These abstractions must be designed carefully, as they must match not only the needs of the developers, but also the capabilities and execution model of the underlying hardware.


==> sections/old/pisacontrol.tex <==
\section{Integrated Data-Plane Control}
\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figures/fault-aware-router.pdf}
\caption {
\exprog architecture. Circles represent operations, with arrows for (possibly delayed) control flow. Shaded objects are data structures.}
\label{fig:router} 
\end{figure}


This section introduces our core mechanisms for enabling control operations in PISA switches. We explain these mechanisms through a driving example: the \exprog, a forwarder with fault detection and routing in the data plane. We are motivated to push network control into the data plane to avoid the inherent latency of solutions where detection and routing are done remotely~\cite{hong2013achieving}, so that our system can react at (or near) the speed of the underlying hardware~\cite{hsu2020contra, katta2016hula}.

The \exprog has three components:

\topheading{Forwarding.} The \exprog looks up a next hop for each packet in an
associative array based on its destination address. Before sending the packet
out, the node checks a second data structure to determine if the next hop is
still reachable. If not, it increments a failure counter.

\topheading{Fault detection.} Concurrent with forwarding, a node also 
regularly pings all of its directly connected neighbors to determine if they
are still reachable.

\topheading{Routing.} Interleaved with the above, each node also periodically
scans its data structures for routes with unreachable next hops. When one is
found, the node queries all of its neighbors to find the shortest alternate route.

% \dl{Should we swap the second and third points here? It seems like Routing relies on Fault Detection to know which things are unreachable}


% \begin{enumerate}

% \item \textbf{Forwarding.} To forward each packet, the \exprog uses the packet's destination address to look up a next hop in an associative data structure. Before sending the packet out, the node checks a second data structure to determine if the next hop is still reachable. If not, it increments a failure counter.
% \item \textbf{Fault detection.} Interleaved with packet forwarding, a node also regularly pings all of its directly connected neighbors to detect link or node failures. When a neighbor responds to a ping, a node records the time of response in its neighbor status map. 
% \item \textbf{Routing.} Concurrent with forwarding and fault detection, each node also periodically scans its routing map to identify destinations that either have no next hop, or a next hop that has become unreachable. When such a destination is found, a node broadcasts a query to all of its neighbors. The neighbors reply with the length of their paths to the destination; the node selects the neighbor with the shortest path length as the destination's next hop.
% \end{enumerate}

\subsection{PISA Programmable Packet Processing}

The target for our \exprog is a PISA switch. The core of a PISA switch,
illustrated in Figure~\ref{fig:execmodel}, is a \emph{programmable line-rate
match-action pipeline}. Line rate demands a tightly
synchronized \emph{feed-forward} design: each pipeline stage has a throughput of one packet per cycle and packets only ever move forward through the pipeline. \emph{Instruction-level parallelism} is also critical for line rate. A packet's header moves through each stage in parallel, as a vector. When the packet header enters a stage, \emph{ternary (TCAM)} and \emph{exact (hash + SRAM)} match-action tables evaluate it to feed \emph{ALU vectors} with instructions to modify header fields. The ``programmable'' aspect of the pipeline is the capability to set table layouts and instructions at compile time, and set table entries from a management CPU at run time.

% A stage reads, but cannot write, these tables. 

% The ``programmable'' aspect of the pipeline is the capability to set table layouts and instructions at compile time and populate tables from the switch CPU at run time. 

% Stages can write SRAM from a packet with \emph{stateful ALUs}
Stages also have \emph{stateful ALUs} (sALUs) for updating local SRAM \emph{register arrays}. Each stateful ALU can read from a single address in
SRAM, perform limited computation, and write back to SRAM or modify metadata associated with the packet. All memory operations done in a pass through the pipeline are  \emph{atomic}~\cite{domino} because of the feed-forward design.

After the match-action ingress pipeline, a packet can be directed to one or more egress pipelines for further processing before transmission.  Alternatively, the packet may be sent through a \emph{dedicated recirculation port} that brings it back to the start of the pipeline for additional processing. 
% The pipeline is provisioned for line rate across all ports, including the dedicated recirculation ports. 
Finally, there are semi-programmable ``\emph{support engines}'' outside of the pipeline: \emph{a multicast engine} to copy packets, a \emph{queue manager} to isolate and shape flows, a \emph{packet generator}
for spawning packets, and \emph{configurable MAC blocks} that can
\emph{dynamically pause queues} based on Priority Flow Control (PFC) frames.

% After the match-action pipeline, a \emph{multicast engine} can create packet copies and a \emph{queue manager} that can isolate and shape flows. A packet can be sent out of a \emph{dedicated recirculation port}, which brings it back to the beginning of the pipeline for additional processing. The pipeline is provisioned to handle line rate across all ports, including the dedicated
% recirculation ports. 

% Finally, there are semi-programmable ``\emph{support engines}'' outside of the pipeline, such a \emph{packet generator}
% for spawning packets and \emph{configurable MAC blocks} that can
% \emph{dynamically pause queues} based on Priority Flow Control (PFC) frames. 


% The target for our \exprog is a PISA switch. The core of a PISA switch, illustrated in Figure~\ref{fig:execmodel}, is a \textbf{line rate pipeline} that serves both external ports and \textbf{internal recirculation ports}. It achieves line rate in part due to \textbf{instruction-level parallel units}. Each stage in the pipeline has multiple \textbf{parallel TCAM lookup tables} that evaluate complex conditions to select instructions that feed \textbf{parallel ALU vectors}. 

% Stages also have \textbf{local persistent memory} that can be updated at line rate using \textbf{stateful ALUs} that perform a limited amount of computation. The pipeline itself is \textbf{feed-forward}: packets only ever move in one direction, so all the memory operations done in a single pass are atomic~\cite{domino}. Finally, outside of the core pipeline, there is a collection of other semi-programmable ``\textbf{support engines}'', such as parsers, deparsers, a multicast engine, and a packet generator.



\subsection{Atomic Control Operations via Packets}
Clearly, PISA pipelines are highly optimized for packet processing. \emph{How can we use them for control applications with shared state, 
multiple threads, and distributed computation? }

\begin{figure}[t]
\includegraphics[width=0.8\linewidth]{figures/execmodel.pdf}
\caption {Interleaving the \exprog's control operations and packet processing in a PISA switch.}
\label{fig:execmodel} 
\end{figure}

% core idea 1: map control operations to packets. 
The key observation is that \emph{control-plane tasks can be broken down into atomic operations that map to individual packets}. For example, we have already described the \exprog's routing component as three atomic operations: checking the status of a single route, answering a single query from a neighbor, and processing a query response. Each of these operations can be performed in a single pass through a PISA pipeline, compiled to a ``slice'' of its parallel ALUs, sALUs, and match-action tables, as illustrated in Figure~\ref{fig:execmodel}. 

% core idea 2: execute operations by interleaving control packets with data packets. 
Once we map individual control operations to packets, we can interleave them with regular data packets, as shown in Figure~\ref{fig:execmodel}. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to the data-plane state using stateful ALUs. 

% Once we map control operations to packets, we can interleave them with data plane packets to form ``threads'', as shown in  Figure~\ref{fig:execmodel}. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to the data plane's state using stateful ALUs. 


\subsection{Fast Control Threads via Recirculation} 
To get from simple control operations that happen instantly to complex control operations that take place over time, e.g., from an operation that scans one route entry to a thread that repeatedly scans an entire route table, we can use packet recirculation. 
We can use recirculation for \emph{serial} processing, by recirculating a control packet multiple times to perform one part of its task in each pass, or we can use it for \emph{parallel} processing, by recirculating multiple control packets back-to-back, each operating on a different chunk of data. 

In either case, using even a small fraction of the pipeline bandwidth gives us blisteringly fast control. For example, in the \exprog, suppose we use \emph{one} of the Tofino's dedicated 100 Gb/s recirculation ports for control operations. That is approximately 100M control operations per second. Assuming each control operation checks a single route, the \exprog could identify all the failed routes in a table with 65K entries in under \ms{1}. This is less than one tenth of the time that it takes a optimized remote control thread~\cite{mantis} to simply \emph{read} the table from the pipeline. Further, this leaves the switch with bandwidth for millions of \emph{other} control operations and \emph{billions} of regular data packets per second. 

\subsection{Scheduled Control via Support Engines}
Of course, the control application may not always \emph{want} control threads to operate at such high rates, or, for that matter, at the same switch. For example, the \exprog needs to \emph{periodically} ping its \emph{neighbors} to check if they are still reachable. 
%
This brings us to the last piece of the puzzle: what components of a PISA switch can we use to schedule the \emph{place} and \emph{time} where control operations execute? 

\heading{Place.} Changing \emph{where} an operation executes is straightforward, assuming that switches have addresses. Since control operations are processed like packets, a switch can schedule an operation at another location by encapsulating the corresponding control packet in an appropriately addressed frame and 
forwarding it just like any other packet. With line-rate multicast engines, we can even schedule an operation at \emph{multiple} locations (such as the fast rerouter pinging all neighboring switches) in a single step.

\heading{Time.} Changing \emph{when} an operation executes is harder. Essentially, we need to buffer a control operation for some amount of time. A simple design would buffer it in a register array along with the time at which it should be executed, and then
scan the array periodically to find operations ready to execute.
However, this approach could consume a large number of stateful ALUs. A simple alternative is to just recirculate a control packet repeatedly until it is ready to execute, but this consumes recirculation bandwitdth. A more efficient mechanism is to use a dedicated queue for delayed control operations, which is paused and periodically released using PFC pause frames from the switch's own packet generator.
% \dl{I'm still confused by this. Perhaps it's my lack of familiarity with the field, but the last line seems like a jargon dump that doesn't explain how it helps (it's also weird that we only mention "pausing" the queue, but not unpausing it. Are we pausing it only for a certain amount of time, after which it automatically restarts?}

% Instead, an efficient way to do this is 
% to put the control packet in a queue that the switch keeps paused by using its traffic 
% generator to send PFC packets to the queue's MAC block. 
% \dl{This last sentence lost me. I'm not sure what it means, or how it compares to the other options we listed}





\OMIT{
\subsection{Mechanisms for Control}
How can we use a PISA pipeline for applications with multiple concurrent control threads, shared state, and distributed computation?

% How can we use these diverse and heterogeneous resources to implement an application like the \exprog that features multiple concurrent control threads that share state and perform distributed computation?  

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/execmodel.pdf}
\caption {Interleaving the \exprog's control operations and packet processing in a PISA switch.}
\label{fig:execmodel} 
\end{figure}

% core idea 1: map control operations to packets. 
The key observation is that \emph{control plane tasks can be broken down into atomic operations that map to individual packets}. For example, we have already described the \exprog's routing component as three atomic operations: checking the status of a single route, answering a single query from a neighbor, and processing a query response. Each of these operations can be performed in a single pass through a PISA pipeline, compiled to a ``slice'' of its parallel ALUs, sALUs and lookup tables, as illustrated in Figure~\ref{fig:execmodel}. 

% Once we map each control operation to a packet, we unlock an overwhelming amount of spare capacity in PISA switches. Bandwidth is spare because of 1) recirculation ports that are typically unused; 2) traffic does not usually arrive at line rate. 

% core idea 2: execute operations by interleaving control packets with data packets. 
Once we map control operations to packets, we can interleave them with data plane packets to execute the control ``threads'', as Figure~\ref{fig:execmodel} illustrates. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to all of the data plane's state. 

Performance is an equally important benefit. Pipeline throughput is so high that we only have to use a small fraction of it for blisteringly fast control. For example, in the \exprog, suppose we use \emph{one} of the Tofino's dedicated 100 Gb/s recirculation ports for control operations. That is approximately 100M control operations per second. Assuming each control operation checks a single route, the \exprog could identify all the failed routes in a table with 65K entries in under \ms{1}. This is less than one tenth of the time that it takes a optimized remote control thread~\cite{mantis} to simply \emph{read} the table from the pipeline. Further, this leaves the PISA switch with bandwidth for millions of \emph{other} control operations and \emph{billions} of data plane packets per second. 

Of course, we may not always \emph{want} our control threads to operate at such high rates. For example, the \exprog periodically pings its neighbors to check if they are still reachable. Generating these pings as fast as possible would consume significant 
bandwidth on links shared by data packets. 

This brings us to the last piece of the puzzle: what components of a PISA switch can we use to change the 
\emph{time} and \emph{place} when/where control operations execute?
\begin{itemize}
	\item Changing an operation's location is straightforward. Since operations are packets, all the switch has to do is forward it towards the appropriate unicast or multicast destination, like any other packet.
	\item Changing \emph{when} an operation executes is much more involved. The most efficient option is to use a somewhat 	obscure switch mechanism: the capability for a switch's pipeline to pause its own egress queues by generating priority flow control (PFC) packets. 
\end{itemize}

}

==> sections/old/pisacontrol2.tex <==
\section{Integrated Data-Plane Control}
\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{figures/fault-aware-router.pdf}
\caption {
\exprog architecture. Circles represent operations, with arrows for (possibly delayed) control flow. Shaded objects are data structures.}
\label{fig:router} 
\end{figure}

\reminder{Might want to rename this to something else instead of fast re-router.}

% why integrate control into the data plane

% how do we integrate control into the data plane

% 



A common design underlies many switch programs, as illustrated by
Figure~\ref{fig:usecases}. Applications \emph{process packets} based on
\emph{persistent state}. Changes in the network or its traffic, for example 
link failures~\reminder{f10}, ephemeral congestion~\reminder{contra}, 
or new flow arrivals~\reminder{jaquen}, trigger \emph{control operations} 
that run concurrently with packet processing and update the 
persistent state to change network behavior.

A driving example illustrates the design concretely. Consider the \exprog, a
packet-processing application with two control operations. 

\topheading{Forwarding.} When a packet arrives, the \exprog looks up its  
next hop in an associative array based on destination address. 
Before sending the packet out, it checks a second associative 
array to determine if the next hop is still reachable. If not, 
it increments a failure counter. 

\topheading{Fault detection.} Concurrent with forwarding, an \exprog node also 
regularly pings all of its directly connected neighbors to determine 
next hop reachability. 

\topheading{(Re-)Routing.} Interleaved with the above operations, 
the \exprog can also scan its data structures for routes with 
unreachable next hops. When a route with an 
unreachable next hops is found, the \exprog node queries 
all of its neighbors to find the shortest alternate route.





This section motivates the integration of these control processes into the
data plane and identifies the enabling mechanisms in today's data-plane
hardware. 

\reminder{Introducing the example might be able to come later -- perhaps 
in the section where we summarize the challenges we face with today's 
languages.}

A driving example helps us understand the details more concretely: 
the \exprog, a simple but representative data-plane application 
with two control operations -- fault detection
and rerouting. Figure~\ref{fig:router} shows the three 
components of the \exprog: 

\topheading{Forwarding.} When a packet arrives, the \exprog looks up its  
next hop in an associative array based on destination address. 
Before sending the packet out, it checks a second associative 
array to determine if the next hop is still reachable. If not, 
it increments a failure counter. 

\topheading{Fault detection.} Concurrent with forwarding, an \exprog node also 
regularly pings all of its directly connected neighbors to determine 
next hop reachability. 

\topheading{(Re-)Routing.} Interleaved with the above operations, 
the \exprog can also scan its data structures for routes with 
unreachable next hops. When a route with an 
unreachable next hops is found, the \exprog node queries 
all of its neighbors to find the shortest alternate route.


\subsection{Low-latency Control}
One of the primary motivations for data-plane integrated 
control is low latency. Traditionally, control 
operations ran on processors 

A diverse range of recent systems have shown that 


integrating control operations 
into the data plane is reduced latency. A diverse range of 
systems have demonstrated that 


Improved performance is the primary motivation for integrated data-plane 
control. A diverse range of recent systems have shown that it can improve 
the latency and throughput of control operations by orders of magnitude, 
and that this translates into improved end-user experience 
and network service scalability. For example: TurboEPC 
shows that in 5G networks, integrating signal handling operations 
into the data plane reduces latency by up to 98\% and 
increases throughput by 107X; load balancers show that 
integrating congestion-mitigation control loops 
into the data plane significantly 




\subsection{Motivating Integrated Control}

Performance is the primary motivation for integrated  data-plane control. It
allows a diverse range of  applications to improve the latency and throughput 
of their control operations by orders of magnitude. This  translates into
improved end-user experience and network service scalability, as  recent work
shows.  

\begin{itemize}
    \item{In 5G mobile cores~\reminder{turboEPC}, 
    integrating signal handling operations into 
    the data plane reduces latency by up to 98\%, enabling 
    faster connection setup and migration for users, 
    and increases throughput by 107X, which improves 
    scalability.}

    \item{Load balancers~\reminder{hula, conga, letitflow} 
    integrate their control loops into the data plane 
    to reduce latency, which enables faster reaction 
    to short-lived congestion events. This, in turn, 
    improves application-level performance metrics 
    such as flow completion times.}

    \item{Security services, such as DDoS defense 
    systems~\reminder{jaqen}} and stateful firewalls 
    (Section~\reminder{sfw}) integrate flow 
    setup operations into the data plane. This lowers 
    their latency and improves throughput

    This 
    reduces latency, which minimizes disruption to 
    non-malicious traffic, and improves throughput, 
    which allows the services to support networks 
    with much higher flow arrival rates.}

    \item{Fault tolerant network services, such as 
    the \exprog and F10~\reminder{f10} integrate 
    failure detection and mitigation operations 
    into the data plane. This lets them react 
    to failures faster, minimizing disruption to 
    affected traffic.}

    \item{}

    enable 
    faster reaction to congestion events, which are 
    often short-lived~\reminder{cite}. 

    and, 
    in turn, improved appl
    lower application-level flow completion times 
    and latency. 



    Load balancers~\reminder{hula} that 
    integrate 

    with control 
    loops 



\subsection{Motivating Integrated Control}
Control operations, such as fault detection and re-routing in the \exprog, 
are traditionally done by a processor external to a switch's data-plane ASIC. 
Performance has motivated recent systems to rethink this design and 
integrate control operations into the data-plane itself. Both the 
latency and throughput of control operations can improve by orders 
of magnitude with data-plane integration. 

\begin{itemize}
    \item {Load balancing. Implementing a load balancer's control 
    loop in the data plane reduces its 

    Load balancing control loops implemented 
    in the data plane enable fast reactions to short-lived congestion 
    events, which in turn improves application-level metrics such as 
    flow completion time.}
    \item {Control operations related to }
    responses to short-lived congestion 
    events, which in turn improves overall }

\subsection{Motivating Integrated Control}
Control operations, such as fault detection and re-routing in the \exprog, 
are traditionally done by a processor external to a switch's data-plane ASIC. 
Performance has motivated many recent systems to rethink this design and 
integrate control operations into the data-plane itself. Both the \emph{latency} 
and \emph{throughput} of control operations can improve by orders 
of magnitude with data-plane integration. 




% inter-node latency
% inter-switch

\paragraph{Latency.} 
The latency of a control operation, or how long it takes to adjust data-plane state in response to a change in the network or its traffic, is important in many applications. For example, in the \exprog, low latency minimizes the application-level disruption caused by link failures. 

Integrating control into the data plane greatly reduces latency by eliminating communication overheads. Consider the \exprog as an example. Detecting and routing around a link failure requires at least two rounds of messages between a switch and its neighbors. If the \exprog's control operations ran as a Linux application on the switch's CPU, the operating system itself would add around \us{400} of latency because unidirectional messaging between Linux socket endpoints takes around \us{100} end-to-end~\footnote{https://www.usenix.org/system/files/conference/atc16/atc16-paper_yasukata.pdf}. A version of the \exprog with control in the data plane would completely avoid these overheads. 


\paragraph{Throughput.}

The throughput of control operations

is also important because it limits how frequently a control operation can adjust data-plane state. 


Data-plane integrated control also eliminates the communication overhead between a switch's ASIC and CPU, such as messaging over a PCIe link which adds at least \us{5} of latency. These overheads impact even single-node applications, and have a large effect when control operations occur in groups. For example, Section~\ref{sec:sfw_eval} finds that for a flow-based stateful firewall, data-plane integrated control can reduce the latency of policy updates by orders of magnitude when new flows from trusted hosts arrive in bursts. 


% in the \exprog, if the control operations were implemented by Linux processes running on the switch's management CPU, 
% Consider a \exprog implementation where the control operations are performed by a Linux process running on the switch's management CPU. 
%  run on the switch CPU 

% Consider a \exprog implementation where the routing process runs on the switch's CPU as a Linux program. Given the failure of link $l$, how long will it take the \exprog to identify a new next hop for all routes that use $l$? 

% % re-route task             &   remote                & integrated         \\
% % check 64K routes          &   ~5us                  & 32us               \\
% % query neighbor            &   200us                 & >1us               \\
% % set new next hop          &   20us                  & 0us                \\
% % total                     &   225us                 & 32us               \\

% Table X compares the latency of a remote re-route operation against a simple integrated variant. Remote control has over 7X higher latency, mostly

% remote and integrated re-route operations, broken down by subtask. 

% versions with remote and integrated control, broken down by task. 
% re-route operation down into individual tasks and compares designs with remote and integrated control. 

% Reading the current route array from the data plane takes around 10us with a highly optimized driver, while scanning the array for all the routes that use $l$ takes around 6.4us assuming 100ns memory operations and 64k routes. The most expensive operation is querying neighbor switches for new routes -- the end-to-end latency between two TCP sockets on adjacent nodes is around 100us~\footnote{https://www.usenix.org/system/files/conference/atc16/atc16-paper_yasukata.pdf}, not counting any application- or control platform overheads. At a minimum, the latency of a re-route operation performed on a switch's management CPU is around 200us. 

% If the reroute operation was in the data plane, the communication overheads, which cause the majority of the latency, would be largely eliminated. The latency between two adjacent switch ASICs is around 0.5us, on average. Scanning the routes array for entries that use $l$ can take longer, around 0.5us per entry in a simple implementation (Section~\ref{mechanism:recirc}). Even so, for 64K entries, this adds up to a total latency of under 40us -- over 5X better than using remote control. 









% This section introduces our core mechanisms for enabling control operations in PISA switches. We explain these mechanisms through a driving example: the \exprog, a forwarder with fault detection and routing in the data plane. We are motivated to push network control into the data plane to avoid the inherent latency of solutions where detection and routing are done remotely~\cite{hong2013achieving}, so that our system can react at (or near) the speed of the underlying hardware~\cite{hsu2020contra, katta2016hula}.

% The \exprog has three components:

% \topheading{Forwarding.} The \exprog looks up a next hop for each packet in an
% associative array based on its destination address. Before sending the packet
% out, the node checks a second data structure to determine if the next hop is
% still reachable. If not, it increments a failure counter.

% \topheading{Fault detection.} Concurrent with forwarding, a node also 
% regularly pings all of its directly connected neighbors to determine if they
% are still reachable.

% \topheading{Routing.} Interleaved with the above, each node also periodically
% scans its data structures for routes with unreachable next hops. When one is
% found, the node queries all of its neighbors to find the shortest alternate route.

% \dl{Should we swap the second and third points here? It seems like Routing relies on Fault Detection to know which things are unreachable}


% \begin{enumerate}

% \item \textbf{Forwarding.} To forward each packet, the \exprog uses the packet's destination address to look up a next hop in an associative data structure. Before sending the packet out, the node checks a second data structure to determine if the next hop is still reachable. If not, it increments a failure counter.
% \item \textbf{Fault detection.} Interleaved with packet forwarding, a node also regularly pings all of its directly connected neighbors to detect link or node failures. When a neighbor responds to a ping, a node records the time of response in its neighbor status map. 
% \item \textbf{Routing.} Concurrent with forwarding and fault detection, each node also periodically scans its routing map to identify destinations that either have no next hop, or a next hop that has become unreachable. When such a destination is found, a node broadcasts a query to all of its neighbors. The neighbors reply with the length of their paths to the destination; the node selects the neighbor with the shortest path length as the destination's next hop.
% \end{enumerate}

\subsection{PISA Programmable Packet Processing}

The target for our \exprog is a PISA switch. The core of a PISA switch,
illustrated in Figure~\ref{fig:execmodel}, is a \emph{programmable line-rate
match-action pipeline}. Line rate demands a tightly
synchronized \emph{feed-forward} design: each pipeline stage has a throughput of one packet per cycle and packets only ever move forward through the pipeline. \emph{Instruction-level parallelism} is also critical for line rate. A packet's header moves through each stage in parallel, as a vector. When the packet header enters a stage, \emph{ternary (TCAM)} and \emph{exact (hash + SRAM)} match-action tables evaluate it to feed \emph{ALU vectors} with instructions to modify header fields. The ``programmable'' aspect of the pipeline is the capability to set table layouts and instructions at compile time, and set table entries from a management CPU at run time.

% A stage reads, but cannot write, these tables. 

% The ``programmable'' aspect of the pipeline is the capability to set table layouts and instructions at compile time and populate tables from the switch CPU at run time. 

% Stages can write SRAM from a packet with \emph{stateful ALUs}
Stages also have \emph{stateful ALUs} (sALUs) for updating local SRAM \emph{register arrays}. Each stateful ALU can read from a single address in
SRAM, perform limited computation, and write back to SRAM or modify metadata associated with the packet. All memory operations done in a pass through the pipeline are  \emph{atomic}~\cite{domino} because of the feed-forward design.

After the match-action ingress pipeline, a packet can be directed to one or more egress pipelines for further processing before transmission.  Alternatively, the packet may be sent through a \emph{dedicated recirculation port} that brings it back to the start of the pipeline for additional processing. 
% The pipeline is provisioned for line rate across all ports, including the dedicated recirculation ports. 
Finally, there are semi-programmable ``\emph{support engines}'' outside of the pipeline: \emph{a multicast engine} to copy packets, a \emph{queue manager} to isolate and shape flows, a \emph{packet generator}
for spawning packets, and \emph{configurable MAC blocks} that can
\emph{dynamically pause queues} based on Priority Flow Control (PFC) frames.

% After the match-action pipeline, a \emph{multicast engine} can create packet copies and a \emph{queue manager} that can isolate and shape flows. A packet can be sent out of a \emph{dedicated recirculation port}, which brings it back to the beginning of the pipeline for additional processing. The pipeline is provisioned to handle line rate across all ports, including the dedicated
% recirculation ports. 

% Finally, there are semi-programmable ``\emph{support engines}'' outside of the pipeline, such a \emph{packet generator}
% for spawning packets and \emph{configurable MAC blocks} that can
% \emph{dynamically pause queues} based on Priority Flow Control (PFC) frames. 


% The target for our \exprog is a PISA switch. The core of a PISA switch, illustrated in Figure~\ref{fig:execmodel}, is a \textbf{line rate pipeline} that serves both external ports and \textbf{internal recirculation ports}. It achieves line rate in part due to \textbf{instruction-level parallel units}. Each stage in the pipeline has multiple \textbf{parallel TCAM lookup tables} that evaluate complex conditions to select instructions that feed \textbf{parallel ALU vectors}. 

% Stages also have \textbf{local persistent memory} that can be updated at line rate using \textbf{stateful ALUs} that perform a limited amount of computation. The pipeline itself is \textbf{feed-forward}: packets only ever move in one direction, so all the memory operations done in a single pass are atomic~\cite{domino}. Finally, outside of the core pipeline, there is a collection of other semi-programmable ``\textbf{support engines}'', such as parsers, deparsers, a multicast engine, and a packet generator.



\subsection{Atomic Control Operations via Packets}
Clearly, PISA pipelines are highly optimized for packet processing. \emph{How can we use them for control applications with shared state, 
multiple threads, and distributed computation? }

\begin{figure}[t]
\includegraphics[width=0.8\linewidth]{figures/execmodel.pdf}
\caption {Interleaving the \exprog's control operations and packet processing in a PISA switch.}
\label{fig:execmodel} 
\end{figure}

% core idea 1: map control operations to packets. 
The key observation is that \emph{control-plane tasks can be broken down into atomic operations that map to individual packets}. For example, we have already described the \exprog's routing component as three atomic operations: checking the status of a single route, answering a single query from a neighbor, and processing a query response. Each of these operations can be performed in a single pass through a PISA pipeline, compiled to a ``slice'' of its parallel ALUs, sALUs, and match-action tables, as illustrated in Figure~\ref{fig:execmodel}. 

% core idea 2: execute operations by interleaving control packets with data packets. 
Once we map individual control operations to packets, we can interleave them with regular data packets, as shown in Figure~\ref{fig:execmodel}. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to the data-plane state using stateful ALUs. 

% Once we map control operations to packets, we can interleave them with data plane packets to form ``threads'', as shown in  Figure~\ref{fig:execmodel}. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to the data plane's state using stateful ALUs. 


\subsection{Fast Control Threads via Recirculation} 
\label{mechanism:recirc}
To get from simple control operations that happen instantly to complex control operations that take place over time, e.g., from an operation that scans one route entry to a thread that repeatedly scans an entire route table, we can use packet recirculation. 
We can use recirculation for \emph{serial} processing, by recirculating a control packet multiple times to perform one part of its task in each pass, or we can use it for \emph{parallel} processing, by recirculating multiple control packets back-to-back, each operating on a different chunk of data. 

In either case, using even a small fraction of the pipeline bandwidth gives us blisteringly fast control. For example, in the \exprog, suppose we use \emph{one} of the Tofino's dedicated 100 Gb/s recirculation ports for control operations. That is approximately 100M control operations per second. Assuming each control operation checks a single route, the \exprog could identify all the failed routes in a table with 65K entries in under \ms{1}. This is less than one tenth of the time that it takes a optimized remote control thread~\cite{mantis} to simply \emph{read} the table from the pipeline. Further, this leaves the switch with bandwidth for millions of \emph{other} control operations and \emph{billions} of regular data packets per second. 

\subsection{Scheduled Control via Support Engines}
Of course, the control application may not always \emph{want} control threads to operate at such high rates, or, for that matter, at the same switch. For example, the \exprog needs to \emph{periodically} ping its \emph{neighbors} to check if they are still reachable. 
%
This brings us to the last piece of the puzzle: what components of a PISA switch can we use to schedule the \emph{place} and \emph{time} where control operations execute? 

\heading{Place.} Changing \emph{where} an operation executes is straightforward, assuming that switches have addresses. Since control operations are processed like packets, a switch can schedule an operation at another location by encapsulating the corresponding control packet in an appropriately addressed frame and 
forwarding it just like any other packet. With line-rate multicast engines, we can even schedule an operation at \emph{multiple} locations (such as the fast rerouter pinging all neighboring switches) in a single step.

\heading{Time.} Changing \emph{when} an operation executes is harder. Essentially, we need to buffer a control operation for some amount of time. A simple design would buffer it in a register array along with the time at which it should be executed, and then
scan the array periodically to find operations ready to execute.
However, this approach could consume a large number of stateful ALUs. A simple alternative is to just recirculate a control packet repeatedly until it is ready to execute, but this consumes recirculation bandwitdth. A more efficient mechanism is to use a dedicated queue for delayed control operations, which is paused and periodically released using PFC pause frames from the switch's own packet generator.
% \dl{I'm still confused by this. Perhaps it's my lack of familiarity with the field, but the last line seems like a jargon dump that doesn't explain how it helps (it's also weird that we only mention "pausing" the queue, but not unpausing it. Are we pausing it only for a certain amount of time, after which it automatically restarts?}

% Instead, an efficient way to do this is 
% to put the control packet in a queue that the switch keeps paused by using its traffic 
% generator to send PFC packets to the queue's MAC block. 
% \dl{This last sentence lost me. I'm not sure what it means, or how it compares to the other options we listed}





\OMIT{
\subsection{Mechanisms for Control}
How can we use a PISA pipeline for applications with multiple concurrent control threads, shared state, and distributed computation?

% How can we use these diverse and heterogeneous resources to implement an application like the \exprog that features multiple concurrent control threads that share state and perform distributed computation?  

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/execmodel.pdf}
\caption {Interleaving the \exprog's control operations and packet processing in a PISA switch.}
\label{fig:execmodel} 
\end{figure}

% core idea 1: map control operations to packets. 
The key observation is that \emph{control plane tasks can be broken down into atomic operations that map to individual packets}. For example, we have already described the \exprog's routing component as three atomic operations: checking the status of a single route, answering a single query from a neighbor, and processing a query response. Each of these operations can be performed in a single pass through a PISA pipeline, compiled to a ``slice'' of its parallel ALUs, sALUs and lookup tables, as illustrated in Figure~\ref{fig:execmodel}. 

% Once we map each control operation to a packet, we unlock an overwhelming amount of spare capacity in PISA switches. Bandwidth is spare because of 1) recirculation ports that are typically unused; 2) traffic does not usually arrive at line rate. 

% core idea 2: execute operations by interleaving control packets with data packets. 
Once we map control operations to packets, we can interleave them with data plane packets to execute the control ``threads'', as Figure~\ref{fig:execmodel} illustrates. This approach to concurrency gives us a powerful and intuitive memory model: each operation has atomic access to all of the data plane's state. 

Performance is an equally important benefit. Pipeline throughput is so high that we only have to use a small fraction of it for blisteringly fast control. For example, in the \exprog, suppose we use \emph{one} of the Tofino's dedicated 100 Gb/s recirculation ports for control operations. That is approximately 100M control operations per second. Assuming each control operation checks a single route, the \exprog could identify all the failed routes in a table with 65K entries in under \ms{1}. This is less than one tenth of the time that it takes a optimized remote control thread~\cite{mantis} to simply \emph{read} the table from the pipeline. Further, this leaves the PISA switch with bandwidth for millions of \emph{other} control operations and \emph{billions} of data plane packets per second. 

Of course, we may not always \emph{want} our control threads to operate at such high rates. For example, the \exprog periodically pings its neighbors to check if they are still reachable. Generating these pings as fast as possible would consume significant 
bandwidth on links shared by data packets. 

This brings us to the last piece of the puzzle: what components of a PISA switch can we use to change the 
\emph{time} and \emph{place} when/where control operations execute?
\begin{itemize}
	\item Changing an operation's location is straightforward. Since operations are packets, all the switch has to do is forward it towards the appropriate unicast or multicast destination, like any other packet.
	\item Changing \emph{when} an operation executes is much more involved. The most efficient option is to use a somewhat 	obscure switch mechanism: the capability for a switch's pipeline to pause its own egress queues by generating priority flow control (PFC) packets. 
\end{itemize}

}

==> sections/old/programming_in_lang_v1.tex <==
\subsection{Programming in \lang}
\lang programs are event driven. The most important elements are \emph{events} and \emph{handlers}. An \textbf{event} is a user-defined data type that describes a recent occurrence. A \textbf{handler} is a segment of code that is bound to an event. Handlers execute automatically when events appear and can generate additional events for later processing.  

\begin{figure}[t]
	\begin{lstlisting}[style=DptBlock,xleftmargin=1.5ex,xrightmargin=.5ex]
	// An IP packet enters or exits the program.
	packet entry event !ip_in!(int<32> dst);
	packet exit event !ip_out!(int<8> egrPort);
	// A request to ensure that the route at idx is valid.
	support event !do_check_route!(int<32> idx);
	// A query from switch s for the path length to dst.
	support event !pLenQ!(int<32> s, int<32> dst);
	// An answer from switch s with its path length to dst.
	support event !pLenA!(int<32> s, int<32> dst, int<8> len);
	// A request to ping all neighboring switches.
	support event !do_ping!(int<32> pingId);
	// A ping from neighbor switch s.
	support event !pingQ!(int<32> s, int<32> pingId);
	// A ping response from neighbor switch s.
	support event !pingA!(int<32> s, int<32> pingId);

	\end{lstlisting}
	\caption{Event declarations in the \exprog.}
	\label{fig:eventdecls}
\end{figure}

\subsubsection{Events} Figure~\ref{fig:eventdecls} shows the event declarations for the \exprog from Section~\ref{sec:motivation}. As we can see, events are qualified and there are two main types: packet events and support events.

% mention that packet events are inlined?
\paragraph{Packet events.} Packet events are the interface between a \lang program and an underlying P4 program. A P4 program transfers control flow to \lang by creating a \textbf{packet entry} event, while a \lang handler generates a \textbf{packet exit} event to return control flow back to P4. Packet entry events are expected to occur at line-rate and are processed immediately -- the \lang compiler inlines their handlers into the P4 program. 

From the perspective of a P4 program, a packet event is just a \lang-generated metadata struct. For the \exprog example, the \lang compiler generates the following P4 structs based on the entry and exit events declared in Figure~\ref{fig:eventdecls}: 

\begin{centering}
\begin{multicols}{2}
\begin{lstlisting}[style=P4Snip]
	struct !dpt_ip_in! {
		bit<32> dst;
	}
	struct !dpt_ip_out! {
		bit<8> egrPort;
	}
\end{lstlisting}
\end{multicols}
\end{centering}
% \reminder{Should this struct be a union?}

A minimal P4 program that wraps the \exprog would populate a global instance of the \code{dpt\_ip\_in} struct for every IP packet that arrives and then call the \lang event dispatcher, which would immediately execute the \code{ip\_in} handler. If the handler finds a route for the packet, it generates a \code{ip\_out}event. The \lang compiler translates this generate statement into P4 code that populates an instance of the \code{dpt\_ip\_out} struct, which is returned to the outer P4 program. 

% (represented as struct in P4), while a \lang handler returns control flow back to P4 by generating an exit event. In the \exprog example, the P4 program generates an \code{ip\_in} event for every IP packet that arrives. If the \code{ip\_in} handler finds an egress port for the packet, it generates a \code{ip\_out} event that includes the selected egress port. 


\heading{Support events.} 
Support events enable background processing to update persistent data structures in a \lang program. Unlike packet events, support events are decoupled from their handling. A support event is not handled immediately, but rather at a runtime-configurable future time in a separate pass through the switch's pipeline. Further, a support event can target the local switch (via recirculation) or a different switch from where it was originally generated. 

By decoupling event generation from handling in this way, support events make it easy to express complex tasks that require inter-node communication or multiple passes through a pipeline. For example, the query and response events in the \exprog (Fig.~\ref{fig:eventdecls}) are all handled and generated on different switches, enabling distributed route computation and fault detection. 

Also, the \exprog uses \code{do\_check\_route(int<32> idx)} to scan through the entire routing table. This event's handler checks the routing entry at \code{idx}, then generates a \code{do\_check\_route} event for \code{idx + 1}. After the last entry is checked, the handler pauses for a configurable amount of time before restarting, by generating a \emph{delayed} event to scan index 0. 

All of the above tasks can be expressed concisely using \lang's support events; its compiler takes care of generating all the necessary P4 code and switch configurations, e.g., for parsing, deparsing, queuing, and delaying events. 

Although support events are powerful, their use of recirculation and network bandwidth places inherent limitations on where they can be used safely in a \lang program. For example, a version of the \exprog that generated a \code{do\_check\_route} event on every packet (i.e., unconditionally inside of the \code{ip\_in} handler) would quickly saturate its recirculation port's bandwidth and queue. In Section~\reminder{X}, we describe how static analysis can identify unsafe event generation to help developers improve their application designs. 


% Event functors
% delay
% locate
% priority (maybe)

\heading{Event functors.}
A \lang programmer specifies when and where an event should be handled using \textbf{event functors}, which are essentially functions that transform events. Table \reminder{X} lists all the event functors built into \lang. 

For example, in the \exprog we can declare a variant of the \code{ping\_neighbors} event that is set to be handled at the local switch in \ms{10} using the \emph{delay} functor.

\begin{centering}
\begin{lstlisting}[style=DptSnip]
	event !delayed_do_ping! = %Event%.delay(do_ping(), 10m);
\end{lstlisting}
\end{centering}

Similarly, we can declare a variant of \code{pingQ} that is multicast to all neighboring switches with the \emph{locate} functor. 

\begin{centering}
\begin{lstlisting}[style=DptSnip]
	event !mc_pingQ! = %Event%.locate(pingQ(|self|), |neighbors|);
\end{lstlisting}
\end{centering}
% technically, we use smlocate here. But I don't want to explain the "sm", so I just dropped it for now. -jps
Here, \code{self} and \code{neighbors} are DPT keywords representing the local switch's ID and the ID of the group of all neighboring switches, \code{pingQ(self)} is an instance of the \code{pingQ} event with its first parameter set to \code{self}, and \code{mc_pingQ} is a multicast instance of \code{pingQ(self)} that will be sent to every switch in \code{neighbors}.

\reminder{We might want an event functor to change the queuing priority of an event. So, for example, support events can have a higher priority so that they never get dropped.}

Event functors are composable. So, for example, we can apply \emph{delay} and then \emph{locate} to set both the time and location where an event will be handled. By default, events target the local switch and are handled as soon as possible (in around \ns{500}, the time of a single packet recirculation).

\heading{Launching support threads.}
\reminder{describe the `main' function, which generates a certain set of events when a \lang program starts. Alternately, describe timers.}

\subsubsection{Handlers}
In \lang, a handler is function that is bound to an event and gets called automatically each time the event occurs. A handler performs a (potentially complex) atomic operation that is executed in a single pass through the physical pipeline. 

% rough proof of atomicity: 
% (1) In an RMT switch, packet processing functions that execute in a single pass through a pipeline are atomic. [cite domino paper]
% (2) In DPT, each packet carries at most 1 event.
% (3) In DPT, an event handler executes in a single pass through the pipeline. 
% (4) By contradition, assume that two events a and b caused a non-atomic execution of 2 handlers. 
% (5) (2) implies that a and b map to two different packets, a' and b'.
% (6) (3) implies that the packet processing functions applied to both a' and b' each execute in a single pass through the pipeline. 
% (7) (4, 5, & 6) imply that there exists a packet processing function that can execute in a single pass, but is not atomic. This contradicts (1).


Handlers are defined in a simple imperative language (Fig.~\ref{fig:grammar}) with constructs that are chosen to balance expressiveness and readability with the processing model of the underlying hardware. The goal is a language that is simple, modular, and familiar, but avoids constructs that would tempt developers into writing handlers that are inherently at odds with the underlying hardware.

Figure \reminder{X} shows an example handler from the \exprog. A handler's name defines the type of event that it processes. The handler in Figure~\reminder{X}, for example, processes events of type \reminder{Y}. A handler also always has the same parameters as its event type. When an event occurs, the event's parameters are passed as arguments to its handler. 

\heading{Statements and expressions.}
The body of a handler contains sequentially executed statements that evaluate expressions. Most statements and expressions have equivalents in common high-level imperative languages. There are two exceptions. First, the \textbf{generate statement}, which generates a new event. Second, the \textbf{hash expression}, which calculates the hash of a list of values using special hash units built into switch hardware. The first argument of a hash expression is the hash function's polynomial.


\reminder{Mention the increased flexibility of an if/else statement in \lang compared to Tofino-P4. More details in Section X.}


\noindent To improve modularity and code reuse, \lang supports two kinds of  subroutines: \textbf{functions} and \textbf{memory operations}. 
%Uses of both can be seen in Figure~\reminder{X}.

\heading{Functions.} Users can declare functions in the top level of a program and call them multiple times from different handlers. Function bodies follow the same grammar as handlers, with the addition of an optional return statement. Functions with return values can be called in the right hand side of a local variable declaration or assignment statement. Function calls can also appear in isolation, in which case the return value is ignored. In either case, function calls are inlined by the compiler. 

\heading{Builtins.} \lang also has several builtin modules with functions that cannot be implemented natively. The simplest builtin module is \code{Sys}, which provides access to intrinsic switch metadata and other miscellaneous functions. For example, \code{Sys.ts} returns the ingress timestamp and \code{Sys.random} returns a random integer.


% Array.new(var_id array, size cell_width, a' num_entries);
% b' value = Array.get(var_id array, a' index);
% Array.set(var_id array, a' index, b' value);
% Array.update(var_id array, a' index, 
%   memop get_memop, b' get_arg, 
%   memop set_memop, b' set_arg);

\begin{table}[t]
\newcommand{\apisig}[1]{\lstinline[style=DptSnip, morekeywords={var_id, size, void, memop}]{#1}}
\centering
\small
\begin{tabularx}{\linewidth}{X X}
\toprule
\textbf{Array Function} & \textbf{Description} \\
\midrule
{\apisig{void Array.!new!(var_id a,}\break\apisig{size w, size n)}} & {Create a new array \emph{a} with \emph{n} entries that each store \emph{w} bits.} \\
\arrayrulecolor{black!50}\midrule

{\apisig{void Array.!set!(var_id a,}\break\apisig{int<n> i, int<w> v)}} 
& {Set the \emph{i'th} cell of \emph{a} to \emph{v} 
\break(\apisig{a[i] := v}).} \\

\arrayrulecolor{black!50}\midrule

{\apisig{int<w> Array.!get!(}\break\apisig{var_id a, int<n> i)}} 
& {Return the \emph{i'th} cell of \emph{a}\break (\apisig{a[i]}).} \\

\arrayrulecolor{black!50}\midrule

{\apisig{int<w> Array.!update!(}\break
\apisig{var_id a, int<n> i,}\break
\apisig{memop getf, int<w> getarg,}\break
\apisig{memop setf, int<w> setarg)}} & {Execute \apisig{getf(a[i],getarg)} and  \apisig{setf(a[i],setarg)} concurrently. Set \apisig{a[i]} to the output of \apisig{setfcn} and return the output of \apisig{get_fcn}.}\\

\arrayrulecolor{black}\bottomrule
\end{tabularx}
\caption{API of \lang's builtin \code{Array} module for operations on persistent global state.}
\label{tab:arrayapi}
\end{table}


\heading{Arrays.}
The most important builtin is the \code{Array} module. \code{Array} provides a library of functions to create and update persistent global state. Table~\ref{tab:arrayapi} summarizes the API and Figure~\reminder{X} shows usage examples. 

\code{Array.new} is called indirectly, via a top level global object declaration, to allocate a new array at compile time. The other Array functions perform computation on elements of the array at runtime. \code{Array.set} and \code{Array.get} are wrappers for the more general \code{Array.update} method. 

\code{Array.update} performs computation on a single cell of an array by concurrently executing two \code{memop}s, syntactically restricted stateful functions. Each \code{memop} reads the value in a cell of the array and the value of a local variable, performs a limited amount of computation, and returns a new value. The first \cell{memop} function passed to \code{Array.update} is a \emph{get} function, whose return value is passed back to the caller of \code{Array.update}. The second \code{memop} is a \emph{set} function, whose return value is written to the memory cell. 


% explaining each statement and expression seems too pedantic.. -jsonch
% \heading{Statements.}
% \begin{itemize}
% 	\item \textbf{Declaration} create a local variable scoped inside of the handler. 
% 	\item \textbf{Assignment} evaluate an expression and bind the resulting values to variables. 
% 	\item \textbf{Call} execute a function, ignoring its return value. 
% 	\item \textbf{Return} evaluate an expression and return it to the function's caller. 
% 	\item \textbf{Selection (if/else)} conditionally execute one of up to two alternate sequences of statements.  
% 	\item \textbf{Generate} generate an event.
% \end{itemize}

% \heading{Expressions.}
% \begin{itemize}
% 	\item \textbf{Value} evaluates to a constant value. 
% 	\item \textbf{Variable} evaluates to the value of a variable. 
% 	\item \textbf{Binary operation} evaluates two expressions to values, then evaluates a binary operation over them. 
% 	\item \textbf{Hash} evaluates all arguments to values, then calculates the hash of the values.

% 	\item \textbf{Assignment} evaluate an expression and bind the resulting values to variables. 
% 	\item \textbf{Call} execute a function, ignoring its return value. 
% 	\item \textbf{Return} evaluate an expression and return it to the function's caller. 
% 	\item \textbf{Selection (if/else)} conditionally execute one of up to two alternate sequences of statements.  
% 	\item \textbf{Generate} generate an event.
% \end{itemize}


\subsubsection{Enabling General-purpose Code}
The constructs of \lang described above make it easier to express sophisticated, general-purpose tasks on linerate reconfigurable hardware. 

To illustrate, consider the ways in which the \exprog benefits from \lang's high level of abstraction. 

\heading{Iteration.} The \exprog's routing and fault detection components run continuous loops that iterate over persistent state.
With \lang, this iteration can be expressed cleanly with recursive support events. 

\heading{Nested conditional branching.} Each component of the \exprog has multiple execution paths that are selected conditionally. These control flows are easy to express with \lang's \code{if/else} statements, which unlike the native P4 statements, can support more complex expressions and arbitrary nesting.

\heading{Structured stateful code.} Multiple components of the \exprog execute the same sequences of stateful operations. in \lang, this code reuse can be naturally abstracted using functions and \code{memop}s.

\heading{Concurrency.} The three components of \exprog's components (forwarding, routing, and fault detection) can be thought of as concurrent threads. \lang's event-based programming model gives developers a natural way to specify how these threads should be interleaved on the underlying hardware, with event functors that provide a simple way to express delayed execution and thread priorities. 

\heading{Distributed computation.} The \exprog's route computation and fault detection threads run distributed algorithms that have one-to-one and one-to-many communication patterns. \lang's remote and multicast events are support these operations directly.  

% \subsubsection{Cost Model}
% Below, we summarize three simple `rules' that a \lang developer can use to estimate the cost of a handler, in terms of how many pipeline stages it requires. 

% \begin{itemize}
% 	\item Branching is free. 
% 	\item Besides branches, every statement in a sequence requires 1 pipeline stage.
% 	% \item Generating a support event consumes 1 packet of recirculation port bandwidth.
% 	\item Memory operations may occasionally cost 2 stages, if many independent branches of a program access the same persistent data structure with different functions. The \lang reports when this occurs. 
% \end{itemize}



\subsection{Language Features}
The constructs of \lang described above make it easier to express sophisticated general-purpose tasks running on line-rate reconfigurable hardware. Below, we describe the features of \lang that achieve a complementary goal: making it easier to debug and improve the designs of such programs. 

\subsubsection{Type checking memory access patterns}
There are inherent restrictions on the patterns in which persistent objects, such as arrays arrays, can be accessed. These restrictions stem from the architecture of the underlying hardware~\cite{domino}. In \lang, the restrictions are encoded into the type system, which uses linear typing to ensure that: 
\begin{itemize}
    \item Each code path of a handler performs at most one update operation on each array. 
    \item All code paths of all handlers access arrays in the same order. 
\end{itemize}

By enforcing these restrictions in the type system, the \lang compiler provides the guarantee that if a program type checks, its memory access pattern is compatible with the underlying architecture. When programs have access patterns that are \emph{not} compatible, identifying this during type checking is also beneficial because type checking occurs at an early stage of compilation. This, in turn, enables error messages that are closer to the source level of abstraction and thus more precise and easier for developers to understand. 

\reminder{Could give an example here.}

Section~\reminder{X} describes \lang's linear type system in more detail. 

\subsubsection{Constraining memory operations}

\code{memops}, which a \lang handler passes to \code{Array.update} to perform computation on persistent state, are a special type of function with grammatical and syntactic restrictions. These restrictions, enumerated in Appendix~\ref{app:grammar},  conservatively approximate the capabilities of the stateful alus in the underlying switch architecture. Their purpose is twofold. First, to provide developers with a precise, simple, and high-level description of the stateful operations that can be supported. Second, to give developers have the guarantee that any syntactically correct \code{memop} will be able to compile to the underlying hardware. 

Although the restrictions represent an additional burden on the developer, the alternative is worse. Consider, for example, if \lang allowed \code{Array.update} to use unrestricted functions instead of \code{memops}. When the developer used a function that was too complex, some phase of compilation would fail. If the developer was lucky, the fault would occur in an early pass of the compiler that could correlate the error with the offending function. As we saw in Section~\ref{sec:motivation}, this is often not the case. But, even in this best case scenario, it would be up to the developer to figure out exactly what all the limitations are, either by trial and error or careful reading of detailed architectural specifications (if available).


\subsubsection{Event generation safety}

\reminder{Left off here 1/1/21}

Describe event generation patterns that are unsafe. (e.g., overload bandwidth of recirculation port or switch-to-switch link)

Describe static analysis passes that can detect them. 

\subsubsection{Behavioral modeling in Python}

Translate to Python. 

Direct translation, easy to read. (list rules)

Can simulate and step through execution. 

Make sure that the logic of the program is correct, which, in combination with the constrained memory operations and strong type checking, gives a developer much higher confidence that their program is correct. 


% \paragraph{Testing Environment}

% \subsection{Multi-stage Data Structures}

% Bloom filters, Sketches, Cuckoo hashing, Flow Caches, Dynamic memory allocation, semaphores.

% Using the core of DPT described above, we can easily implement more sophisticated custom data structures. 

% \paragraph{Bloom Filters}
% \paragraph{Cuckoo Hash Tables}
% \paragraph{Flow Caches}
% \paragraph{Dynamic Memory Allocation}
% \paragraph{Semaphores}


